The VLA/ALMA Nascent Disk and Multiplicity (VANDAM) Survey of Orion Protostars. A Statistical Characterization of Class 0 and I Protostellar Disks

We have conducted a survey of 328 protostars in the Orion molecular clouds with ALMA at 0.87 mm at a resolution of $\sim$0.1" (40 au), including observations with the VLA at 9 mm toward 148 protostars at a resolution of $\sim$0.08" (32 au). This is the largest multi-wavelength survey of protostars at this resolution by an order of magnitude. We use the dust continuum emission at 0.87 mm and 9 mm to measure the dust disk radii and masses toward the Class 0, Class I, and Flat Spectrum protostars, characterizing the evolution of these disk properties in the protostellar phase. The mean dust disk radii for the Class 0, Class I, and Flat Spectrum protostars are 44.9$^{+5.8}_{-3.4}$, 37.0$^{+4.9}_{-3.0}$, and 28.5$^{+3.7}_{-2.3}$ au, respectively, and the mean protostellar dust disk masses are 25.9$^{+7.7}_{-4.0}$, 14.9$^{+3.8}_{-2.2}$, 11.6$^{+3.5}_{-1.9}$ Earth masses, respectively. The decrease in dust disk masses is expected from disk evolution and accretion, but the decrease in disk radii may point to the initial conditions of star formation not leading to the systematic growth of disk radii or that radial drift is keeping the dust disk sizes small. At least 146 protostellar disks (35% out of 379 detected 0.87 mm continuum sources plus 42 non-detections) have disk radii greater than 50 au in our sample. These properties are not found to vary significantly between different regions within Orion. The protostellar dust disk mass distributions are systematically larger than that of Class II disks by a factor of $>$4, providing evidence that the cores of giant planets may need to at least begin their formation during the protostellar phase.

==> tab11.tex <==
\begin{deluxetable}{lll}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Median Dust Disk Masses for Star Forming Regions and Samples}

\tablehead{\colhead{Region} & \colhead{Dust Disk Mass} & \colhead{Reference} \\
                            &  \colhead{(M$_{\earth}$)}
}
\startdata
Protostellar Disk Samples\\
\hline   
Orion Class 0       & 25.7 (52.5) & 1\\
Orion Class I       & 15.6 (15.2) & 1\\
Orion Flat Spectrum & 13.8 (22.0) & 1\\
Orion Class 0  (T = 20K, $\kappa$=3.45)     & 127.1 (187.9) & 1\\
Orion Class I  (T = 20K, $\kappa$=3.45)      & 48.3 (39.0) & 1\\
Orion Flat Spectrum (T = 20K, $\kappa$=3.45)  & 39.6 (44.0) & 1\\
\hline
Oph Class I         & 3.5  & 2\\
Oph Flat Spectrum   & 2.1  & 2\\
Taurus              & 50.0 & 3\\
Perseus Class 0     & 633.8 & 4\\
Perseus Class I     & 137.3 & 4\\
\hline
Proto-planetary Disk Samples\\
\hline
Chameleon            & 1.8 & 5\\
Lupus                & 3.5 & 6\\
Taurus               & 3.3 & 7\\
Oph                  & 0.6 & 2\\
Orion Nebula Cluster & 0.8 & 8\\
Upper Scorpius       & 0.3 & 9\\
%Orion Molecular Cloud 2 &  & 10\\
\enddata
\tablecomments{The medians for the non-multiples in Orion are given in the parentheses.
References: This work (1), \citet{williams2019} (2), \citet{sheehan2017b} (3),
\citet{tychoniec2018} (4), \citet{pascucci2016} (5), \citet{ansdell2016} (6), \citet{tripathi2017} (7),
\citet{eisner2018} (8), and \citet{barenfeld2016} (9).}
\end{deluxetable}


==> tab2-short.tex <==
\startlongtable
\begin{deluxetable}{llllllll}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{ALMA Fields}

\tablehead{\colhead{Field} & \colhead{RA} & \colhead{Dec.} & \colhead{L$_{bol}$} & \colhead{T$_{bol}$} & \colhead{Distance} & \colhead{Class} & \colhead{Sources} \\
                           & \colhead{(J2000)} & \colhead{(J2000)}   & \colhead{(L$_{\sun}$)}  & \colhead{(K)}  & \colhead{(pc)}          &                   
}
\startdata
\input{table-alma-fields-short.tex}
\enddata
\tablecomments{The fields HOPS-395, HOPS-406, and HOPS-408 were observed twice due to a different target
name being assigned to the same position. The duplicate fields have a `-d' appended to their field name.
The field names that begin with S13 are taken from \citet{stutz2013}, which identified them as potential 
protostellar sources. However, no sources were detected within the S13 fields.}
\end{deluxetable}




==> tab3-short.tex <==
\startlongtable
\begin{deluxetable}{lcll}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{VLA Observations}

\tablehead{\colhead{Field(s)} & \colhead{Number of Fields} & \colhead{Date} & \colhead{Calibrators}\\
                              &                             & \colhead{(UT)} & \colhead{Bandpass, Flux, Complex Gain}
}

\startdata
\input{table-vla-obslog-short.tex}
\enddata
\tablecomments{
The standard observation length was 2.5 hours, and we achieved $\sim$1 hour on-source. For the observations
with Number of sources listed as 2, the observation length was 4 hours, and we were able to still reach
$\sim$1 hr on source for each source in the SB. Observing efficiency is improved due to sharing the
flux and bandpass calibration in addition to the fixed 10 minute overhead at the start of the observation.
}
\end{deluxetable}




==> tab4-short.tex <==
\startlongtable
\begin{deluxetable}{llllllll}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{VLA Fields}

\tablehead{\colhead{Field} & \colhead{RA} & \colhead{Dec.} & \colhead{L$_{bol}$} & \colhead{T$_{bol}$} & \colhead{Distance} & \colhead{Class} & \colhead{Sources} \\
                           & \colhead{(J2000)} & \colhead{(J2000)}   & \colhead{(L$_{\sun}$)}  & \colhead{(K)}  & \colhead{(pc)}          &                   
}
\startdata
\input{table-vla-fields-short.tex}
\enddata
\end{deluxetable}




==> tab6-short.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllllllllllll}
\tabletypesize{\tiny}
\tablewidth{0pt}
\tablecaption{ALMA Source Properties}

\tablehead{\colhead{Source} & \colhead{RA}      & \colhead{Dec.}      & \colhead{ALMA Field}     & \colhead{$\Delta\phi_{A}$}  &  \colhead{VLA Field} & \colhead{$\Delta\phi_{V}$} &\colhead{Class}      & \colhead{F$_{\nu}$} & \colhead{Peak F$_{\nu}$} & \colhead{RMS} & \colhead{Decon. Size} & \colhead{Decon. PA}\\
                            & \colhead{(J2000)} & \colhead{(J2000)}   &                          & \colhead{(\arcsec)}            &                      & \colhead{(\arcsec)}          &                     & \colhead{(mJy)}      & \colhead{(mJy~bm$^{-1}$)} & \colhead{(mJy)}      & \colhead{(\arcsec)}    & \colhead{(\degr)}         
}
\startdata
\input{table-alma-data-short.tex}
\enddata
\tablecomments{Table 6 is published in its entirety in the machine-readable format.
      A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}
\end{longrotatetable}


==> tab7-short.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllllllllllll}
\tabletypesize{\tiny}
\tablewidth{0pt}
\tablecaption{VLA Source Properties}

\tablehead{\colhead{Source} & \colhead{RA}      & \colhead{Dec.}      & \colhead{ALMA Field}     & \colhead{$\Delta\phi_{A}$}  &  \colhead{VLA Field} & \colhead{$\Delta\phi_{V}$}  & \colhead{Class}     & \colhead{F$_{\nu}$} & \colhead{Peak F$_{\nu}$} & \colhead{RMS} & \colhead{Decon. Size} & \colhead{Decon. PA}\\
                            & \colhead{(J2000)} & \colhead{(J2000)}   &                          & \colhead{(\arcsec)}            &                      & \colhead{(\arcsec)}           &                     & \colhead{(mJy)}      &\colhead{(mJy~bm$^{-1}$)} &\colhead{($\mu$Jy)} & \colhead{(\arcsec)}    & \colhead{(\degr)}     
}
\startdata
\input{table-vla-data-short.tex}
\enddata
\end{deluxetable}
\tablecomments{Table 7 is published in its entirety in the machine-readable format.
      A portion is shown here for guidance regarding its form and content.}
\end{longrotatetable}


==> tab8-short.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllllllllllll}
\tabletypesize{\tiny}
\tablewidth{0pt}
\tablecaption{ALMA and VLA Derived Parameters}

\tablehead{\colhead{Source} & \colhead{L$_{bol}$}  & \colhead{T$_{bol}$} & \colhead{Class} & \colhead{R$_{26\sigma,ALMA}$} & \colhead{R$_{2\sigma,VLA}$} & \colhead{M$_{D,ALMA}$} & \colhead{M$_{D,VLA}$} & \colhead{Q$_{ALMA}$} & \colhead{Q$_{VLA}$} & \colhead{Sp. Index} & \colhead{Sp. Index}\\
                            & \colhead{(L$_{\sun}$)} & \colhead{(K)}     &                 & \colhead{(au)}            & \colhead{(au)}           & \colhead{(M$_{\earth}$)}  & \colhead{(M$_{\earth}$)}  & & &  \colhead{(0.87 - 9~mm)} &  \colhead{(8.1 - 10~mm)}   
}
\startdata
\input{table-alma-vla-data-derived-short.tex}
\enddata
\end{deluxetable}
\tablecomments{Table 8 is published in its entirety in the machine-readable format.
 A portion is shown here for guidance regarding its form and content.}
\end{longrotatetable}


==> table-alma-data-short.tex <==
HH270VLA1-A & 05:51:34.587 & +02:56:46.01 & HH270VLA1 & 1.1 & HH270VLA1 & 2.3 & 0    & 18.90$\pm$0.68 & 14.79 & 0.32 & 0.08$\times$0.03 & 143.9\\
HH270VLA1-B & 05:51:34.600 & +02:56:45.88 & HH270VLA1 & 0.9 & HH270VLA1 & 2.2 & 0    & 17.71$\pm$0.73 & 12.90 & 0.32 & 0.10$\times$0.04 & 141.2\\
HH270mms1-B & 05:51:22.632 & +02:56:06.80 & HH270mms1 & 0.1 & HH270mms  & 13.4 & I    & 9.57$\pm$2.56 & 7.06 & 1.06 & 0.08$\times$0.07 & 2.7\\
HH270mms1-A & 05:51:22.717 & +02:56:04.98 & HH270mms1 & 2.2 & HH270mms  & 11.7 & I    & 258.94$\pm$5.25 & 68.77 & 1.11 & 0.27$\times$0.14 & 87.4\\
HH270mms2  & 05:51:22.572 & +02:55:43.16 & HH270mms2 & 0.4 & HH270mms  & 10.3 & Flat & 75.44$\pm$2.17 & 14.20 & 0.38 & 0.25$\times$0.20 & 47.3\\
HH111MMS-B & 05:51:46.066 & +02:48:30.80 & HH111mms  & 2.8 & HH111mms  & 3.0 & I    & 25.44$\pm$4.56 & 21.91 & 2.43 & 0.07$\times$0.04 & 146.2\\
HH111MMS-A & 05:51:46.253 & +02:48:29.65 & HH111mms  & 0.2 & HH111mms  & 0.0 & I    & 694.09$\pm$15.68 & 101.69 & 2.28 & 0.55$\times$0.17 & 7.6\\
HOPS-367   & 05:54:36.287 & +01:53:54.06 & HOPS-367  & 0.4 & None      & \nodata & I    & 1.01$\pm$0.21 & 0.94 & 0.22 & \nodata & \nodata\\
HOPS-7     & 05:54:20.057 & +01:50:42.64 & HOPS-7    & 0.2 & HOPS-7    & 0.2 & 0    & 44.49$\pm$1.21 & 15.08 & 0.31 & 0.26$\times$0.07 & 154.8\\
HOPS-6     & \nodata & \nodata & HOPS-6    & 0.0 & None      & \nodata & I    & $\leq$0.67 & $\leq$0.67 & 0.22 & \nodata & \nodata\\


==> table-alma-fields-short.tex <==
HH270VLA1      & 05:51:34.626 & +02:56:45.02 & 7.0 & 32.0 &  430.1 & 0    &  2\\
HH270mms1      & 05:51:22.631 & +02:56:06.73 & 8.3 & 72.0 &  405.7 & I    &  2\\
HH270mms2      & 05:51:22.559 & +02:55:42.78 & 4.7 & 249.0 &  413.3 & Flat &  1\\
HH111mms       & 05:51:46.238 & +02:48:29.65 & 23.0 & 78.0 &  410.6 & I    &  2\\
HOPS-367       & 05:54:36.259 & +01:53:54.02 & 0.0 & 249.4 &  354.9 & I    &  1\\
HOPS-7         & 05:54:20.045 & +01:50:42.75 & 0.5 & 58.0 &  357.1 & 0    &  1\\
HOPS-6         & 05:54:18.411 & +01:49:03.43 & 0.1 & 112.5 &  357.0 & I    &  0\\
HOPS-5         & 05:54:32.163 & +01:48:07.16 & 0.4 & 187.1 &  354.6 & I    &  1\\
HOPS-4         & 05:54:53.765 & +01:47:09.96 & 0.4 & 203.3 &  351.6 & I    &  1\\
HOPS-354       & 05:54:24.253 & +01:44:19.39 & 6.6 & 34.8 &  355.4 & 0    &  1\\


==> table-alma-vla-data-derived-short.tex <==
HH270VLA1-A & 7.3 & 32.0 & 0    & 30.7$\pm$10.0 & 28.5$\pm$10.0 & 13.4$\pm$0.5 & 242.4$\pm$19.0 & 27.696 & 1.585 & 1.9$\pm$0.07 & 1.0$\pm$0.63\\
HH270VLA1-C & 7.3 & 32.0 & 0    & \nodata & 39.1$\pm$10.0 & \nodata & 528.6$\pm$29.0 & \nodata & 0.688 & \nodata & -0.4$\pm$0.48\\
HH270VLA1-B & 7.3 & 32.0 & 0    & 36.5$\pm$10.0 & \nodata      & 12.6$\pm$0.5 & 87.8$\pm$6.0 & 28.387 & \nodata & 2.3$\pm$0.07 & 3.1$\pm$0.52\\
HH270mms1-B & 7.7 & 72.0 & I    & 27.9$\pm$18.9 & \nodata & 6.0$\pm$1.6 & $\leq$21.8 & 62.810 & \nodata & \nodata & \nodata \\
HH270mms1-A & 7.7 & 72.0 & I    & 92.3$\pm$10.0 & 32.4$\pm$10.0 & 161.3$\pm$3.4 & 793.9$\pm$23.1 & 1.729 & 0.467 & 2.4$\pm$0.06 & 1.9$\pm$0.23\\
HH270mms2  & 4.6 & 249.0 & Flat & 87.4$\pm$10.0 & \nodata & 56.7$\pm$1.6 & $\leq$24.9 & 5.804 & \nodata & \nodata & \nodata \\
HH111MMS-B & 22.0 & 78.0 & I    & 23.0$\pm$14.6 & 14.3$\pm$10.0 & 12.2$\pm$2.3 & 118.5$\pm$11.1 & 24.084 & 2.761 & 2.1$\pm$0.11 & 1.9$\pm$0.79\\
HH111MMS-A & 22.0 & 78.0 & I    & 192.2$\pm$10.0 & 44.3$\pm$10.0 & 332.0$\pm$7.5 & 1504.3$\pm$22.1 & 0.508 & 0.180 & 2.5$\pm$0.06 & 1.3$\pm$0.12\\
HOPS-367   & 0.0 & 249.4 & I    & \nodata      & \nodata & 2.8$\pm$0.6 & \nodata & \nodata & \nodata & \nodata & \nodata \\
HOPS-7     & 0.4 & 58.0 & 0    & 78.8$\pm$10.0 & 20.0$\pm$10.0 & 52.4$\pm$1.4 & 177.8$\pm$27.7 & 13.549 & 4.863 & 2.5$\pm$0.09 & 2.7$\pm$1.41\\


==> table-alma-vla-data.tex <==
HH270VLA1-A & 05:51:34.587 & +02:56:46.01 & HH270VLA1 & 1.1 & HH270VLA1 & 2.3 & 7.3 & 32.0 & 0    & 18.90$\pm$0.68 & 0.24$\pm$0.02  & 0.08$\times$0.03 & 143.9 & 16.8 & 0.08$\times$0.03 & 143.0 & 15.6 & 0.004$\pm$0.000 & 0.073$\pm$0.006 & 1.9 & 0.07\\
HH270VLA1-C & 05:51:34.595 & +02:56:45.89 & HH270VLA1 & 1.0 & HH270VLA1 & 2.2 & 7.3 & 32.0 & 0    & -99.00$\pm$-99.00 & 0.53$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.11$\times$0.09 & 50.3 & 21.4 & -99.000$\pm$-99.000 & 0.159$\pm$0.009 & -99.0 & -99.00\\
HH270VLA1-B & 05:51:34.600 & +02:56:45.88 & HH270VLA1 & 0.9 & HH270VLA1 & 2.2 & 7.3 & 32.0 & 0    & 17.71$\pm$0.73 & 0.09$\pm$0.01  & 0.10$\times$0.04 & 141.2 & 20.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.026$\pm$0.002 & 2.3 & 0.07\\
HH270mms1-B & 05:51:22.632 & +02:56:06.80 & HH270mms1 & 0.1 & HH270mms  & 13.4 & 7.7 & 72.0 & I    & 9.57$\pm$2.56 & 0.02$\pm$0.02  & 0.08$\times$0.07 & 2.7 & 16.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.007$\pm$0.007 & 2.5 & 0.45\\
HH270mms1-A & 05:51:22.717 & +02:56:04.98 & HH270mms1 & 2.2 & HH270mms  & 11.7 & 7.7 & 72.0 & I    & 258.94$\pm$5.25 & 0.91$\pm$0.03  & 0.27$\times$0.14 & 87.4 & 53.6 & 0.09$\times$0.06 & 98.6 & 18.8 & 0.048$\pm$0.001 & 0.238$\pm$0.007 & 2.4 & 0.06\\
HH270mms2  & 05:51:22.572 & +02:55:43.16 & HH270mms2 & 0.4 & HH270mms  & 10.3 & 4.6 & 249.0 & Flat & 75.44$\pm$2.17 & 0.02$\pm$0.02  & 0.25$\times$0.20 & 47.3 & 49.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.017$\pm$0.000 & 0.007$\pm$0.007 & 3.4 & 0.43\\
HH111MMS-B & 05:51:46.066 & +02:48:30.80 & HH111mms  & 2.8 & HH111mms  & 3.0 & 22.0 & 78.0 & I    & 25.44$\pm$4.56 & 0.17$\pm$0.02  & 0.07$\times$0.04 & 146.2 & 13.2 & 0.04$\times$0.02 & 82.0 & 8.2 & 0.004$\pm$0.001 & 0.036$\pm$0.003 & 2.1 & 0.11\\
HH111MMS-A & 05:51:46.253 & +02:48:29.65 & HH111mms  & 0.2 & HH111mms  & 0.0 & 22.0 & 78.0 & I    & 694.09$\pm$15.68 & 2.18$\pm$0.03  & 0.55$\times$0.17 & 7.6 & 110.2 & 0.13$\times$0.09 & 7.5 & 25.4 & 0.100$\pm$0.002 & 0.451$\pm$0.007 & 2.5 & 0.06\\
HOPS-367   & 05:54:36.287 & +01:53:54.06 & HOPS-367  & 0.4 & None      & -99.0 & 0.0 & 249.4 & I    & 1.01$\pm$0.21 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-7     & 05:54:20.057 & +01:50:42.64 & HOPS-7    & 0.2 & HOPS-7    & 0.2 & 0.4 & 58.0 & 0    & 44.49$\pm$1.21 & 0.12$\pm$0.02  & 0.26$\times$0.07 & 154.8 & 52.0 & 0.07$\times$0.06 & 149.5 & 13.2 & 0.016$\pm$0.000 & 0.053$\pm$0.008 & 2.5 & 0.09\\
HOPS-6     & \nodata & \nodata & HOPS-6    & 0.0 & None      & -99.0 & 0.0 & 112.5 & I    & 0.67$\pm$0.67 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-5     & 05:54:32.163 & +01:48:07.08 & HOPS-5    & 0.1 & None      & -99.0 & 0.3 & 187.1 & I    & 44.43$\pm$1.17 & -99.00$\pm$-99.00  & 0.19$\times$0.09 & 12.6 & 37.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.017$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-4     & 05:54:53.789 & +01:47:09.70 & HOPS-4    & 0.4 & None      & -99.0 & 0.3 & 203.3 & I    & 4.30$\pm$0.59 & -99.00$\pm$-99.00  & 0.12$\times$0.08 & 12.6 & 24.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-354   & 05:54:24.262 & +01:44:19.91 & HOPS-354  & 0.5 & HOPS-354  & 0.5 & 4.7 & 34.8 & 0    & 54.97$\pm$1.08 & 1.90$\pm$0.02  & 0.08$\times$0.07 & 158.6 & 16.2 & 0.08$\times$0.03 & 61.3 & 15.4 & 0.009$\pm$0.000 & 0.434$\pm$0.004 & 1.4 & 0.06\\
HOPS-3     & 05:54:56.963 & +01:42:56.23 & HOPS-3    & 0.1 & None      & -99.0 & 0.4 & 467.5 & Flat & 39.49$\pm$1.46 & -99.00$\pm$-99.00  & 0.41$\times$0.09 & 36.8 & 82.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-2     & 05:54:09.137 & +01:42:51.70 & HOPS-2    & 0.3 & None      & -99.0 & 0.4 & 356.5 & I    & 8.95$\pm$0.52 & -99.00$\pm$-99.00  & 0.07$\times$0.04 & 162.4 & 14.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-1     & 05:54:12.347 & +01:42:35.48 & HOPS-1    & 0.2 & HOPS-1    & 0.2 & 1.1 & 72.6 & I    & 14.09$\pm$0.53 & 0.15$\pm$0.02  & 0.06$\times$0.03 & 2.5 & 12.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.049$\pm$0.005 & 2.0 & 0.08\\
HOPS-346   & \nodata & \nodata & HOPS-346  & 0.0 & None      & -99.0 & 0.3 & 649.5 & Flat & 0.67$\pm$6.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.004 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
2MJ05474500+0038418-A & 05:47:44.999 & +00:38:41.89 & None      & -99.0 & HOPS-406  & 31.3 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.85$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.09$\times$0.06 & 58.8 & 17.6 & -99.000$\pm$-99.000 & 0.423$\pm$0.011 & -99.0 & -99.00\\
2MJ05474500+0038418-B & 05:47:44.960 & +00:38:41.82 & None      & -99.0 & HOPS-406  & 30.8 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.11$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.053$\pm$0.004 & -99.0 & -99.00\\
HOPS-345   & 05:47:38.966 & +00:38:36.21 & HOPS-345  & 0.2 & None      & -99.0 & 0.5 & 219.4 & I    & 68.33$\pm$1.90 & -99.00$\pm$-99.00  & 0.34$\times$0.13 & 81.8 & 68.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.032$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-406   & 05:47:43.434 & +00:38:21.31 & HOPS-406  & 1.6 & HOPS-406  & 1.6 & 0.5 & 24.6 & 0    & 15.47$\pm$0.69 & 0.04$\pm$0.01  & 0.14$\times$0.11 & 64.2 & 28.2 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.007$\pm$0.000 & 0.024$\pm$0.005 & 2.5 & 0.11\\
HOPS-344   & 05:47:24.735 & +00:37:34.83 & HOPS-344  & 0.4 & None      & -99.0 & 0.1 & 408.2 & I    & 5.92$\pm$0.89 & -99.00$\pm$-99.00  & 0.38$\times$0.04 & 66.3 & 75.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-343   & 05:47:59.041 & +00:35:32.83 & HOPS-343  & 0.2 & HOPS-343  & 0.2 & 4.1 & 82.1 & I    & 6.88$\pm$0.72 & 0.08$\pm$0.02  & 0.15$\times$0.11 & 120.8 & 30.8 & 0.09$\times$0.07 & 2.9 & 18.4 & 0.002$\pm$0.000 & 0.028$\pm$0.005 & 1.9 & 0.11\\
HOPS-342   & 05:47:57.108 & +00:35:27.12 & HOPS-342  & 0.4 & HOPS-343  & 29.4 & 0.3 & 312.6 & I    & 1.33$\pm$0.21 & 0.03$\pm$0.03  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.020$\pm$0.020 & 1.6 & 0.44\\
HOPS-404   & 05:48:07.714 & +00:33:51.83 & HOPS-404  & 1.3 & HOPS-404  & 1.3 & 1.0 & 26.1 & 0    & 306.36$\pm$6.16 & 2.66$\pm$0.04  & 0.16$\times$0.16 & 144.2 & 32.8 & 0.13$\times$0.12 & 64.8 & 26.8 & 0.117$\pm$0.002 & 1.321$\pm$0.018 & 2.0 & 0.06\\
HOPS-340   & 05:47:01.311 & +00:26:23.04 & HOPS-340  & 1.6 & HOPS-340-341 & 3.7 & 1.9 & 40.6 & 0    & 57.35$\pm$0.95 & 0.39$\pm$0.02  & 0.11$\times$0.07 & 99.7 & 22.8 & 0.06$\times$0.05 & 86.8 & 12.0 & 0.018$\pm$0.000 & 0.165$\pm$0.009 & 2.1 & 0.07\\
HOPS-341   & 05:47:00.914 & +00:26:21.49 & HOPS-341  & 1.4 & HOPS-340-341 & 2.5 & 2.2 & 39.4 & 0    & 27.97$\pm$1.06 & 0.14$\pm$0.02  & 0.15$\times$0.09 & 145.8 & 29.8 & 0.08$\times$0.00 & 172.5 & 15.2 & 0.008$\pm$0.000 & 0.056$\pm$0.008 & 2.3 & 0.09\\
HOPS-338-B & 05:46:57.302 & +00:23:57.97 & HOPS-338  & 7.8 & HOPS-338  & 7.8 & 0.2 & 53.7 & 0    & 46.14$\pm$1.20 & 0.18$\pm$0.04  & 0.42$\times$0.08 & 9.1 & 83.8 & 0.26$\times$0.12 & 2.9 & 51.6 & 0.028$\pm$0.001 & 0.131$\pm$0.030 & 2.4 & 0.12\\
HOPS-338-A & 05:46:57.356 & +00:23:50.43 & HOPS-338  & 0.3 & HOPS-338  & 0.3 & 0.2 & 53.7 & 0    & 9.34$\pm$0.51 & 0.02$\pm$0.02  & 0.07$\times$0.04 & 15.6 & 13.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & 0.017$\pm$0.017 & 2.6 & 0.43\\
HOPS-337   & 05:46:55.092 & +00:23:34.55 & HOPS-337  & 0.1 & HOPS-338  & 37.2 & 0.9 & 128.8 & I    & 30.44$\pm$0.76 & 0.15$\pm$0.01  & 0.09$\times$0.05 & 45.6 & 18.8 & 0.03$\times$0.02 & 145.4 & 5.0 & 0.012$\pm$0.000 & 0.074$\pm$0.004 & 2.3 & 0.07\\
HOPS-336   & 05:46:02.278 & +00:23:30.60 & HOPS-336  & 0.1 & None      & -99.0 & 0.0 & 164.6 & I    & 1.12$\pm$0.22 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-393   & 05:46:42.485 & +00:23:01.13 & HOPS-393  & 0.2 & None      & -99.0 & 0.1 & 250.5 & I    & 4.96$\pm$0.62 & -99.00$\pm$-99.00  & 0.15$\times$0.05 & 32.8 & 29.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-335   & \nodata & \nodata & HOPS-335  & 0.0 & None      & -99.0 & 0.5 & 81.1 & I    & 0.68$\pm$0.68 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-366-B & 05:47:04.009 & +00:22:10.45 & HOPS-366  & 0.4 & HOPS-361  & 29.9 & 6.8 & 292.2 & I    & 16.94$\pm$0.84 & 0.12$\pm$0.01  & 0.06$\times$0.03 & 62.6 & 11.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.035$\pm$0.002 & 2.1 & 0.07\\
HOPS-366-A & 05:47:04.003 & +00:22:10.33 & HOPS-366  & 0.4 & HOPS-361  & 29.8 & 6.8 & 292.2 & I    & 38.37$\pm$0.85 & 0.52$\pm$0.02  & 0.06$\times$0.04 & 67.2 & 11.8 & 0.09$\times$0.06 & 162.0 & 18.6 & 0.008$\pm$0.000 & 0.158$\pm$0.007 & 1.8 & 0.06\\
HOPS-361-H & 05:47:05.125 & +00:22:01.46 & None      & -99.0 & HOPS-361  & 19.3 & 503.1 & 69.0 & 0    & -99.00$\pm$-99.00 & 0.28$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.08$\times$0.06 & 18.0 & 16.6 & -99.000$\pm$-99.000 & 0.029$\pm$0.002 & -99.0 & -99.00\\
HOPS-361-G-A & 05:47:05.367 & +00:21:50.53 & HOPS-361  & 11.7 & HOPS-361  & 11.7 & 503.1 & 69.0 & 0    & 31.59$\pm$1.24 & 0.46$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.09$\times$0.06 & 44.3 & 18.2 & 0.002$\pm$0.000 & 0.048$\pm$0.002 & 1.8 & 0.07\\
HOPS-361-G-B & 05:47:05.451 & +00:21:50.08 & HOPS-361  & 12.4 & HOPS-361  & 12.4 & 503.1 & 69.0 & 0    & 18.99$\pm$1.24 & 0.28$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.07$\times$0.04 & 13.3 & 13.8 & 0.001$\pm$0.000 & 0.029$\pm$0.002 & 1.8 & 0.07\\
HOPS-361-C-B & 05:47:04.625 & +00:21:47.88 & HOPS-361  & 5.5 & HOPS-361  & 5.5 & 503.1 & 69.0 & 0    & -99.00$\pm$-99.00 & 0.38$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.039$\pm$0.001 & -99.0 & -99.00\\
HOPS-361-C & 05:47:04.631 & +00:21:47.85 & HOPS-361  & 5.4 & HOPS-361  & 5.4 & 503.1 & 69.0 & 0    & 883.40$\pm$9.15 & 2.21$\pm$0.02  & 0.47$\times$0.19 & 130.1 & 95.0 & 0.14$\times$0.04 & 6.7 & 27.0 & 0.061$\pm$0.001 & 0.228$\pm$0.002 & 2.6 & 0.06\\
HOPS-361-B & 05:47:04.755 & +00:21:45.45 & HOPS-361  & 2.6 & HOPS-361  & 2.6 & 503.1 & 69.0 & 0    & 94.38$\pm$2.56 & 1.76$\pm$0.02  & 0.06$\times$0.05 & 174.4 & 11.2 & 0.07$\times$0.04 & 55.5 & 14.8 & 0.006$\pm$0.000 & 0.182$\pm$0.002 & 1.7 & 0.06\\
HOPS-361-A & 05:47:04.783 & +00:21:42.86 & HOPS-361  & 0.1 & HOPS-361  & 0.1 & 503.1 & 69.0 & 0    & 606.35$\pm$6.28 & 5.45$\pm$0.03  & 0.26$\times$0.15 & 14.4 & 52.6 & 0.10$\times$0.07 & 64.4 & 20.2 & 0.042$\pm$0.000 & 0.563$\pm$0.003 & 2.0 & 0.06\\
HOPS-361-E & 05:47:04.624 & +00:21:41.30 & HOPS-361  & 2.8 & HOPS-361  & 2.7 & 503.1 & 69.0 & 0    & 29.41$\pm$4.23 & 0.15$\pm$0.02  & 0.15$\times$0.11 & 111.9 & 29.2 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.015$\pm$0.002 & 2.3 & 0.10\\
HOPS-361-F & 05:47:04.967 & +00:21:40.74 & HOPS-361  & 3.6 & HOPS-361  & 3.6 & 503.1 & 69.0 & 0    & 6.63$\pm$1.24 & 0.09$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.000$\pm$0.000 & 0.010$\pm$0.001 & 1.8 & 0.11\\
HOPS-361-D & 05:47:04.317 & +00:21:38.04 & HOPS-361  & 8.4 & HOPS-361  & 8.4 & 503.1 & 69.0 & 0    & 71.27$\pm$4.34 & 0.30$\pm$0.02  & 0.17$\times$0.09 & 43.1 & 34.8 & 0.09$\times$0.06 & 50.9 & 18.6 & 0.005$\pm$0.000 & 0.031$\pm$0.002 & 2.3 & 0.07\\
HOPS-392   & 05:46:16.505 & +00:21:35.75 & HOPS-392  & 0.5 & None      & -99.0 & 0.1 & 62.4 & 0    & 1.68$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-334   & \nodata & \nodata & HOPS-334  & 0.0 & None      & -99.0 & 0.1 & 506.7 & Flat & 0.70$\pm$0.70 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-361-J & 05:47:04.525 & +00:21:23.89 & None      & -99.0 & HOPS-361  & 19.3 & 503.1 & 69.0 & 0    & -99.00$\pm$-99.00 & 0.10$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.011$\pm$0.001 & -99.0 & -99.00\\
HOPS-347   & 05:47:15.947 & +00:21:22.89 & HOPS-347  & 1.2 & HOPS-347  & 1.2 & 0.6 & 33.5 & 0    & 22.19$\pm$0.72 & 0.15$\pm$0.02  & 0.12$\times$0.04 & 43.0 & 23.2 & 0.06$\times$0.02 & 49.4 & 12.4 & 0.010$\pm$0.000 & 0.087$\pm$0.010 & 2.1 & 0.08\\
HOPS-361-I & 05:47:04.246 & +00:21:22.70 & None      & -99.0 & HOPS-361  & 21.7 & 503.1 & 69.0 & 0    & -99.00$\pm$-99.00 & 0.13$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.013$\pm$0.001 & -99.0 & -99.00\\
HOPS-365   & 05:47:10.613 & +00:21:13.71 & HOPS-365  & 0.4 & None      & -99.0 & 20.3 & 160.3 & I    & 128.03$\pm$2.34 & -99.00$\pm$-99.00  & 0.11$\times$0.10 & 101.4 & 21.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.021$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-359   & 05:47:24.840 & +00:20:59.39 & HOPS-359  & 0.7 & HOPS-359  & 0.7 & 10.5 & 36.7 & 0    & 139.95$\pm$3.18 & 0.24$\pm$0.02  & 0.17$\times$0.15 & 3.6 & 34.0 & 0.06$\times$0.04 & 10.8 & 11.6 & 0.027$\pm$0.001 & 0.065$\pm$0.005 & 2.7 & 0.07\\
HOPS-333   & \nodata & \nodata & HOPS-333  & 0.0 & HOPS-359  & 28.9 & 0.2 & 240.9 & Flat & 0.64$\pm$0.64 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.025$\pm$0.025 & 1.2 & 0.61\\
HOPS-391   & \nodata & \nodata & HOPS-391  & 0.0 & HOPS-347  & 35.2 & 0.1 & 58.1 & 0    & 0.65$\pm$0.65 & 0.04$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & 0.036$\pm$0.036 & 1.2 & 0.61\\
HOPS-390   & 05:47:32.455 & +00:20:21.64 & HOPS-390  & 0.3 & HOPS-390  & 0.3 & 3.4 & 54.3 & 0    & 110.82$\pm$2.67 & 0.18$\pm$0.03  & 0.47$\times$0.12 & 15.8 & 93.8 & 0.13$\times$0.08 & 23.0 & 26.8 & 0.029$\pm$0.001 & 0.064$\pm$0.011 & 2.8 & 0.10\\
HOPS-364-B & 05:47:36.554 & +00:20:06.00 & HOPS-364  & 0.3 & None      & -99.0 & 34.3 & 96.7 & I    & 16.18$\pm$1.34 & -99.00$\pm$-99.00  & 0.05$\times$0.03 & 8.4 & 10.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-364-A & 05:47:36.563 & +00:20:05.92 & HOPS-364  & 0.3 & None      & -99.0 & 34.3 & 96.7 & I    & 95.47$\pm$1.99 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 177.7 & 19.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-331   & 05:46:28.337 & +00:19:49.33 & HOPS-331  & 0.3 & HOPS-407  & 22.4 & 0.4 & 82.5 & Flat & 22.39$\pm$0.66 & 0.06$\pm$0.01  & 0.07$\times$0.06 & 30.0 & 15.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.012$\pm$0.000 & 0.041$\pm$0.005 & 2.5 & 0.08\\
HOPS-407   & 05:46:28.251 & +00:19:27.96 & HOPS-407  & 1.0 & HOPS-407  & 1.0 & 0.7 & 26.8 & 0    & 62.20$\pm$1.76 & 0.14$\pm$0.02  & 0.18$\times$0.14 & 173.6 & 36.0 & 0.10$\times$0.04 & 162.2 & 20.0 & 0.025$\pm$0.001 & 0.072$\pm$0.009 & 2.6 & 0.08\\
HOPS-329   & 05:47:01.601 & +00:17:58.92 & HOPS-329  & 0.1 & None      & -99.0 & 2.6 & 89.2 & I    & 4.96$\pm$0.88 & -99.00$\pm$-99.00  & 0.16$\times$0.11 & 18.6 & 32.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-326   & 05:46:39.554 & +00:04:16.87 & HOPS-326  & 0.5 & HOPS-326  & 0.5 & 0.6 & 58.8 & 0    & 1.65$\pm$0.21 & 0.03$\pm$0.03  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.017$\pm$0.017 & 1.7 & 0.44\\
HOPS-325   & 05:46:39.199 & +00:01:12.31 & HOPS-325  & 2.8 & HOPS-325  & 2.8 & 6.5 & 49.2 & 0    & 80.10$\pm$1.46 & 0.24$\pm$0.02  & 0.10$\times$0.09 & 119.0 & 19.2 & 0.05$\times$0.03 & 65.7 & 10.6 & 0.018$\pm$0.000 & 0.074$\pm$0.005 & 2.5 & 0.07\\
HOPS-363-A & 05:46:43.122 & +00:00:52.35 & HOPS-363  & 0.1 & None      & -99.0 & 23.4 & 367.6 & Flat & 29.62$\pm$0.72 & -99.00$\pm$-99.00  & 0.08$\times$0.05 & 25.7 & 15.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-363-B & 05:46:43.132 & +00:00:52.25 & HOPS-363  & 0.3 & None      & -99.0 & 23.4 & 367.6 & Flat & 2.16$\pm$0.31 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-324   & 05:46:37.566 & +00:00:33.83 & HOPS-324  & 0.4 & HOPS-325  & 48.3 & 2.3 & 89.9 & I    & 2.71$\pm$0.24 & 0.07$\pm$0.07  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.027$\pm$0.027 & 1.6 & 0.43\\
HOPS-389-B & 05:46:46.604 & +00:00:29.52 & HOPS-389  & 6.8 & HOPS-389  & 6.8 & 6.2 & 42.8 & 0    & 4.79$\pm$0.33 & 0.03$\pm$0.03  & 0.06$\times$0.03 & 33.4 & 12.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.010$\pm$0.010 & 2.2 & 0.43\\
HOPS-389-A & 05:46:47.019 & +00:00:27.07 & HOPS-389  & 0.1 & HOPS-389  & 0.1 & 6.2 & 42.8 & 0    & 19.72$\pm$0.67 & 0.12$\pm$0.02  & 0.10$\times$0.07 & 50.1 & 19.6 & 0.06$\times$0.02 & 151.1 & 12.8 & 0.004$\pm$0.000 & 0.038$\pm$0.006 & 2.2 & 0.09\\
HOPS-323-A & 05:46:47.697 & +00:00:25.27 & HOPS-323  & 0.1 & HOPS-389  & 10.3 & 10.3 & 82.9 & I    & 44.48$\pm$0.75 & 0.24$\pm$0.02  & 0.07$\times$0.05 & 30.9 & 14.0 & 0.04$\times$0.01 & 51.4 & 7.2 & 0.009$\pm$0.000 & 0.064$\pm$0.005 & 2.2 & 0.07\\
HOPS-323-B & 05:46:47.667 & +00:00:24.81 & HOPS-323  & 0.6 & HOPS-389  & 9.9 & 10.3 & 82.9 & I    & 81.35$\pm$1.48 & 0.10$\pm$0.02  & 0.30$\times$0.08 & 50.7 & 59.4 & 0.04$\times$0.03 & 130.4 & 8.0 & 0.016$\pm$0.000 & 0.027$\pm$0.005 & 2.9 & 0.10\\
HOPS-322   & 05:46:46.517 & +00:00:16.09 & HOPS-322  & 0.4 & HOPS-389  & 13.3 & 0.5 & 71.3 & I    & 19.99$\pm$0.72 & 0.09$\pm$0.01  & 0.17$\times$0.06 & 105.8 & 35.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.009$\pm$0.000 & 0.052$\pm$0.006 & 2.3 & 0.08\\
HOPS-321   & 05:46:33.172 & +00:00:02.03 & HOPS-321  & 0.2 & HOPS-321  & 0.2 & 3.9 & 78.6 & I    & 5.38$\pm$1.32 & 0.05$\pm$0.01  & 0.30$\times$0.22 & 59.1 & 59.8 & 0.05$\times$0.03 & 139.1 & 10.4 & 0.001$\pm$0.000 & 0.017$\pm$0.003 & 2.0 & 0.14\\
HOPS-403   & 05:46:27.906 & -00:00:52.15 & HOPS-403  & 2.9 & HOPS-403  & 2.9 & 4.3 & 43.9 & 0    & 584.08$\pm$12.81 & 3.18$\pm$0.06  & 0.39$\times$0.38 & 64.0 & 77.2 & 0.30$\times$0.29 & 73.1 & 61.0 & 0.144$\pm$0.003 & 1.081$\pm$0.022 & 2.2 & 0.06\\
HOPS-373-A & 05:46:31.099 & -00:02:33.02 & HOPS-373  & 6.6 & HOPS-373  & 6.6 & 5.5 & 36.9 & 0    & 103.83$\pm$1.63 & 0.25$\pm$0.02  & 0.19$\times$0.17 & 135.8 & 38.4 & 0.09$\times$0.06 & 1.0 & 18.4 & 0.024$\pm$0.000 & 0.079$\pm$0.007 & 2.6 & 0.07\\
HOPS-373-B & 05:46:30.905 & -00:02:35.19 & HOPS-373  & 3.3 & HOPS-373  & 3.3 & 5.5 & 36.9 & 0    & 92.21$\pm$0.95 & 0.07$\pm$0.01  & 0.10$\times$0.09 & 144.3 & 19.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.021$\pm$0.000 & 0.021$\pm$0.004 & 3.1 & 0.10\\
HOPS-320   & 05:46:14.212 & -00:05:26.81 & HOPS-320  & 0.1 & None      & -99.0 & 0.5 & 87.0 & I    & 5.68$\pm$0.76 & -99.00$\pm$-99.00  & 0.17$\times$0.12 & 56.2 & 34.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-388   & 05:46:13.140 & -00:06:04.90 & HOPS-388  & 0.4 & None      & -99.0 & 27.6 & 321.9 & Flat & 209.34$\pm$4.42 & -99.00$\pm$-99.00  & 0.20$\times$0.19 & 130.5 & 39.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.031$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-319   & \nodata & \nodata & HOPS-319  & 0.0 & None      & -99.0 & 0.0 & 464.2 & I    & 0.61$\pm$0.61 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-318   & 05:46:13.521 & -00:08:55.93 & HOPS-318  & 0.7 & None      & -99.0 & 0.2 & 312.6 & Flat & 1.45$\pm$0.22 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-386-C & 05:46:08.923 & -00:09:56.12 & HOPS-386  & 9.1 & HOPS-317  & 42.7 & 23.4 & 147.4 & I    & 30.89$\pm$1.01 & 0.27$\pm$0.03  & 0.16$\times$0.06 & 125.6 & 31.8 & 0.11$\times$0.06 & 27.8 & 22.2 & 0.005$\pm$0.000 & 0.059$\pm$0.006 & 2.0 & 0.07\\
HOPS-387-A & 05:46:07.838 & -00:09:59.59 & HOPS-387  & 1.3 & HOPS-317  & 40.5 & 5.6 & 118.3 & I    & 111.89$\pm$1.50 & 0.36$\pm$0.03  & 0.27$\times$0.11 & 42.9 & 54.4 & 0.16$\times$0.06 & 24.7 & 31.2 & 0.025$\pm$0.000 & 0.114$\pm$0.009 & 2.5 & 0.07\\
HOPS-386-B & 05:46:08.429 & -00:10:00.52 & HOPS-386  & 2.4 & HOPS-317  & 38.1 & 23.4 & 147.4 & I    & 39.83$\pm$3.26 & 0.05$\pm$0.05  & 0.45$\times$0.31 & 68.3 & 90.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & 0.011$\pm$0.011 & 2.9 & 0.43\\
HOPS-387-B & 05:46:07.856 & -00:10:01.30 & HOPS-387  & 0.5 & HOPS-317  & 38.8 & 5.6 & 118.3 & I    & 29.84$\pm$0.82 & 0.22$\pm$0.02  & 0.10$\times$0.06 & 76.2 & 20.6 & 0.07$\times$0.04 & 59.3 & 13.0 & 0.007$\pm$0.000 & 0.069$\pm$0.006 & 2.1 & 0.07\\
HOPS-386-A & 05:46:08.487 & -00:10:03.05 & HOPS-386  & 0.4 & HOPS-317  & 35.5 & 23.4 & 147.4 & I    & 102.94$\pm$0.95 & 0.74$\pm$0.02  & 0.12$\times$0.07 & 56.8 & 23.4 & 0.06$\times$0.05 & 20.0 & 11.0 & 0.016$\pm$0.000 & 0.163$\pm$0.004 & 2.1 & 0.06\\
HOPS-317-A & 05:46:08.597 & -00:10:38.49 & HOPS-317  & 0.1 & HOPS-317  & 0.1 & 4.9 & 47.5 & 0    & 65.69$\pm$2.27 & 0.17$\pm$0.04  & 0.10$\times$0.09 & 48.3 & 19.0 & 0.19$\times$0.07 & 113.8 & 38.6 & 0.015$\pm$0.001 & 0.056$\pm$0.013 & 2.5 & 0.12\\
HOPS-317-B & 05:46:08.376 & -00:10:43.65 & HOPS-317  & 6.0 & HOPS-317  & 6.0 & 4.9 & 47.5 & 0    & 1348.63$\pm$13.06 & 2.16$\pm$0.05  & 0.74$\times$0.52 & 92.2 & 148.4 & 0.21$\times$0.14 & 133.7 & 42.6 & 0.318$\pm$0.003 & 0.706$\pm$0.017 & 2.8 & 0.06\\
HOPS-402   & 05:46:10.031 & -00:12:16.88 & HOPS-402  & 0.9 & HOPS-402  & 0.9 & 0.6 & 24.2 & 0    & 419.42$\pm$9.81 & 1.77$\pm$0.06  & 0.43$\times$0.29 & 58.7 & 86.4 & 0.33$\times$0.24 & 28.3 & 66.4 & 0.187$\pm$0.004 & 0.997$\pm$0.033 & 2.3 & 0.06\\
HOPS-401   & 05:46:07.724 & -00:12:21.25 & HOPS-401  & 1.2 & HOPS-401  & 1.2 & 0.6 & 26.0 & 0    & 128.94$\pm$2.93 & 0.25$\pm$0.02  & 0.21$\times$0.16 & 176.9 & 41.2 & 0.11$\times$0.07 & 168.4 & 21.8 & 0.056$\pm$0.001 & 0.136$\pm$0.009 & 2.7 & 0.07\\
HOPS-316   & \nodata & \nodata & HOPS-316  & 0.0 & HOPS-316-358 & 2.8 & 4.3 & 55.2 & 0    & 0.78$\pm$0.78 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.009$\pm$0.009 & 1.5 & 0.61\\
HOPS-358-A & 05:46:07.257 & -00:13:30.22 & HOPS-358  & 0.5 & HOPS-316-358 & 4.5 & 25.8 & 41.7 & 0    & 223.77$\pm$2.06 & 0.54$\pm$0.02  & 0.38$\times$0.10 & 81.2 & 75.2 & 0.12$\times$0.03 & 66.0 & 23.4 & 0.033$\pm$0.000 & 0.116$\pm$0.005 & 2.6 & 0.06\\
HOPS-358-B & 05:46:07.331 & -00:13:43.50 & HOPS-358  & 13.7 & HOPS-316-358 & 17.8 & 25.8 & 41.7 & 0    & 416.33$\pm$2.89 & 0.90$\pm$0.05  & 0.29$\times$0.27 & 127.0 & 57.4 & 0.17$\times$0.15 & 139.9 & 34.2 & 0.062$\pm$0.000 & 0.192$\pm$0.011 & 2.6 & 0.06\\
HOPS-385   & 05:46:04.775 & -00:14:16.68 & HOPS-385  & 0.4 & None      & -99.0 & 12.1 & 377.1 & Flat & 67.34$\pm$1.26 & -99.00$\pm$-99.00  & 0.08$\times$0.07 & 6.1 & 15.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.012$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-315   & 05:46:03.635 & -00:14:49.56 & HOPS-315  & 0.4 & None      & -99.0 & 6.4 & 180.3 & I    & 145.38$\pm$2.77 & -99.00$\pm$-99.00  & 0.13$\times$0.12 & 165.0 & 25.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.032$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HH212mms   & 05:43:51.408 & -01:02:53.16 & HH212mms  & 0.0 & HH212mms  & 0.3 & 13.5 & 53.0 & 0    & 186.00$\pm$4.13 & 0.60$\pm$0.02  & 0.22$\times$0.10 & 118.6 & 44.8 & 0.10$\times$0.04 & 112.4 & 20.0 & 0.031$\pm$0.001 & 0.143$\pm$0.005 & 2.5 & 0.06\\
HOPS-312-A & 05:43:05.690 & -01:15:54.59 & HOPS-312  & 0.4 & HOPS-312  & 0.4 & 0.7 & 46.7 & 0    & 24.11$\pm$0.65 & 0.17$\pm$0.01  & 0.07$\times$0.05 & 117.8 & 13.6 & 0.05$\times$0.02 & 116.0 & 9.8 & 0.009$\pm$0.000 & 0.085$\pm$0.006 & 2.1 & 0.07\\
HOPS-312-B & 05:43:05.705 & -01:15:54.83 & HOPS-312  & 0.6 & HOPS-312  & 0.5 & 0.7 & 46.7 & 0    & 9.37$\pm$0.67 & 0.11$\pm$0.01  & 0.08$\times$0.05 & 139.9 & 15.8 & 0.06$\times$0.05 & 2.6 & 12.6 & 0.004$\pm$0.000 & 0.053$\pm$0.007 & 1.9 & 0.09\\
HOPS-400-A & 05:42:45.246 & -01:16:13.62 & HOPS-400  & 0.6 & HOPS-400  & 0.6 & 2.9 & 35.0 & 0    & 123.09$\pm$5.49 & 0.65$\pm$0.01  & 0.14$\times$0.13 & 100.2 & 27.6 & 0.05$\times$0.05 & 49.0 & 10.6 & 0.032$\pm$0.001 & 0.229$\pm$0.005 & 2.2 & 0.06\\
HOPS-400-B & 05:42:45.257 & -01:16:14.03 & HOPS-400  & 0.4 & HOPS-400  & 0.4 & 2.9 & 35.0 & 0    & 602.79$\pm$16.49 & 2.02$\pm$0.05  & 0.44$\times$0.41 & 18.5 & 87.4 & 0.26$\times$0.24 & 16.6 & 51.4 & 0.157$\pm$0.004 & 0.716$\pm$0.018 & 2.4 & 0.06\\
HOPS-311   & 05:43:03.056 & -01:16:29.32 & HOPS-311  & 0.5 & None      & -99.0 & 2.8 & 383.0 & Flat & 68.19$\pm$1.56 & -99.00$\pm$-99.00  & 0.17$\times$0.11 & 43.2 & 34.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.018$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-310   & 05:42:27.677 & -01:20:01.33 & HOPS-310  & 0.3 & HOPS-310  & 0.3 & 13.5 & 51.8 & 0    & 473.56$\pm$9.55 & 1.48$\pm$0.02  & 0.29$\times$0.15 & 45.7 & 57.6 & 0.09$\times$0.07 & 34.1 & 18.4 & 0.079$\pm$0.002 & 0.352$\pm$0.005 & 2.5 & 0.06\\
J054227.77-012902.2 & 05:42:27.764 & -01:20:02.20 & HOPS-310  & 1.8 & HOPS-310  & 1.8 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.23$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.104$\pm$0.006 & -99.0 & -99.00\\
HOPS-305   & 05:41:45.386 & -01:51:56.82 & HOPS-305  & 0.2 & None      & -99.0 & 0.9 & 300.7 & Flat & 39.97$\pm$1.12 & -99.00$\pm$-99.00  & 0.13$\times$0.12 & 51.6 & 26.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.014$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-357-B & 05:41:39.143 & -01:52:07.29 & HOPS-357  & 0.7 & None      & -99.0 & 14.3 & 628.2 & Flat & 29.63$\pm$1.62 & -99.00$\pm$-99.00  & 0.06$\times$0.04 & 23.2 & 11.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-357-A & 05:41:39.128 & -01:52:07.45 & HOPS-357  & 0.5 & None      & -99.0 & 14.3 & 628.2 & Flat & 121.81$\pm$2.37 & -99.00$\pm$-99.00  & 0.12$\times$0.09 & 30.2 & 24.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.020$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-384-region-H & 05:41:45.902 & -01:54:11.17 & None      & -99.0 & HOPS-384  & 43.5 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.76$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.055$\pm$0.002 & -99.0 & -99.00\\
2M05414611-0154147 & 05:41:46.123 & -01:54:14.99 & None      & -99.0 & HOPS-384  & 42.9 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 2.49$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 1.120$\pm$0.012 & -99.0 & -99.00\\
2M05414482-0154251 & 05:41:44.828 & -01:54:25.31 & None      & -99.0 & HOPS-384  & 22.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.79$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.05$\times$0.04 & 66.0 & 9.6 & -99.000$\pm$-99.000 & 0.353$\pm$0.015 & -99.0 & -99.00\\
HOPS-384-region-I & 05:41:43.167 & -01:54:25.42 & None      & -99.0 & HOPS-384  & 24.0 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.10$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.008$\pm$0.002 & -99.0 & -99.00\\
HOPS-384-region-F & 05:41:43.087 & -01:54:26.27 & None      & -99.0 & HOPS-384  & 24.1 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.61$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.06$\times$0.04 & 52.7 & 11.8 & -99.000$\pm$-99.000 & 0.044$\pm$0.003 & -99.0 & -99.00\\
HOPS-384-region-D & 05:41:45.524 & -01:54:27.14 & None      & -99.0 & HOPS-384  & 28.1 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 1.09$\pm$0.12  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.20$\times$0.17 & 97.6 & 39.8 & -99.000$\pm$-99.000 & 0.079$\pm$0.009 & -99.0 & -99.00\\
2M05414550-0154286 & 05:41:45.490 & -01:54:28.92 & None      & -99.0 & HOPS-384  & 26.6 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.09$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.040$\pm$0.009 & -99.0 & -99.00\\
2M05414580-0154297-A & 05:41:45.810 & -01:54:30.05 & None      & -99.0 & HOPS-384  & 29.9 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 51.39$\pm$0.05  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.07$\times$0.07 & 25.5 & 14.6 & -99.000$\pm$-99.000 & 23.107$\pm$0.021 & -99.0 & -99.00\\
2M05414580-0154297-B & 05:41:45.805 & -01:54:30.30 & None      & -99.0 & HOPS-384  & 29.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 1.89$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.07$\times$0.04 & 99.9 & 13.2 & -99.000$\pm$-99.000 & 0.850$\pm$0.018 & -99.0 & -99.00\\
HOPS-384-region-G & 05:41:43.915 & -01:54:34.09 & HOPS-384  & 11.3 & HOPS-384  & 11.3 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.65$\pm$0.13  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.31$\times$0.14 & 162.7 & 62.6 & -99.000$\pm$-99.000 & 0.047$\pm$0.009 & -99.0 & -99.00\\
2M05414325-0154343 & 05:41:43.248 & -01:54:34.35 & HOPS-384  & 16.5 & HOPS-384  & 16.5 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.09$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.039$\pm$0.012 & -99.0 & -99.00\\
2M05414483-0154357 & 05:41:44.842 & -01:54:35.98 & HOPS-384  & 14.6 & HOPS-384  & 14.6 & -99.0 & -99.0 & \nodata & 68.48$\pm$1.82 & 0.52$\pm$0.07  & 0.14$\times$0.08 & 93.9 & 28.0 & 0.11$\times$0.10 & 166.0 & 21.8 & 0.024$\pm$0.001 & 0.234$\pm$0.031 & 2.1 & 0.08\\
HOPS-384-B & 05:41:44.016 & -01:54:43.14 & HOPS-384  & 2.2 & HOPS-384  & 2.2 & 1404.9 & 51.9 & 0    & 127.66$\pm$5.41 & 0.03$\pm$0.03  & 0.73$\times$0.18 & 34.9 & 145.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & 0.002$\pm$0.002 & 3.6 & 0.43\\
2M05414138-0154445 & 05:41:41.390 & -01:54:44.75 & None      & -99.0 & HOPS-384  & 40.4 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.27$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.122$\pm$0.011 & -99.0 & -99.00\\
HOPS-384-A-B & 05:41:44.140 & -01:54:45.97 & HOPS-384  & 1.2 & HOPS-384  & 1.2 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.20$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.015$\pm$0.001 & -99.0 & -99.00\\
HOPS-384-A & 05:41:44.135 & -01:54:46.06 & HOPS-384  & 1.2 & HOPS-384  & 1.2 & 1404.9 & 51.9 & 0    & 200.18$\pm$1.60 & 1.39$\pm$0.04  & 0.10$\times$0.07 & 60.2 & 21.0 & 0.06$\times$0.04 & 16.3 & 11.2 & 0.010$\pm$0.000 & 0.101$\pm$0.003 & 2.1 & 0.06\\
2M05414512-0154470 & 05:41:45.126 & -01:54:47.19 & HOPS-384  & 15.7 & HOPS-384  & 15.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.32$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.04$\times$0.04 & 24.2 & 8.8 & -99.000$\pm$-99.000 & 0.145$\pm$0.015 & -99.0 & -99.00\\
HOPS-384-C & 05:41:44.252 & -01:54:55.53 & HOPS-384  & 10.7 & HOPS-384  & 10.7 & 1404.9 & 51.9 & 0    & 41.48$\pm$2.91 & 0.03$\pm$0.03  & 0.21$\times$0.17 & 62.6 & 41.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.002$\pm$0.002 & 3.2 & 0.43\\
HOPS-384-region-E & 05:41:45.735 & -01:54:57.97 & None      & -99.0 & HOPS-384  & 27.9 & 1404.9 & 51.9 & 0    & -99.00$\pm$-99.00 & 0.94$\pm$0.20  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.39$\times$0.24 & 102.5 & 78.8 & -99.000$\pm$-99.000 & 0.068$\pm$0.014 & -99.0 & -99.00\\
2M05414418-0155203 & 05:41:44.184 & -01:55:20.52 & None      & -99.0 & HOPS-384  & 35.5 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.16$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.08$\times$0.03 & 160.1 & 16.0 & -99.000$\pm$-99.000 & 0.071$\pm$0.018 & -99.0 & -99.00\\
HOPS-304-A & 05:41:45.954 & -01:56:26.59 & HOPS-304  & 0.5 & None      & -99.0 & 4.0 & 354.9 & Flat & 24.59$\pm$0.64 & -99.00$\pm$-99.00  & 0.05$\times$0.04 & 37.7 & 10.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-304-B & 05:41:45.912 & -01:56:26.80 & HOPS-304  & 0.8 & None      & -99.0 & 4.0 & 354.9 & Flat & 13.10$\pm$0.59 & -99.00$\pm$-99.00  & 0.04$\times$0.03 & 133.2 & 7.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-303   & 05:42:02.649 & -02:07:45.98 & HOPS-303  & 0.5 & HOPS-303  & 0.6 & 1.4 & 43.2 & 0    & 199.12$\pm$4.30 & 0.67$\pm$0.02  & 0.24$\times$0.19 & 164.0 & 47.6 & 0.10$\times$0.04 & 80.2 & 19.0 & 0.062$\pm$0.001 & 0.278$\pm$0.010 & 2.4 & 0.06\\
HOPS-299   & 05:41:44.610 & -02:16:06.63 & HOPS-299  & 0.5 & None      & -99.0 & 18.6 & 277.0 & I    & 5.00$\pm$0.86 & -99.00$\pm$-99.00  & 0.13$\times$0.09 & 135.2 & 26.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-300   & 05:41:24.212 & -02:16:06.66 & HOPS-300  & 0.2 & None      & -99.0 & 0.7 & 93.7 & I    & 5.19$\pm$0.56 & -99.00$\pm$-99.00  & 0.10$\times$0.08 & 101.7 & 20.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-298-A & 05:41:37.192 & -02:17:17.35 & HOPS-298  & 0.4 & None      & -99.0 & 29.4 & 169.3 & I    & 278.64$\pm$5.82 & -99.00$\pm$-99.00  & 0.19$\times$0.12 & 3.1 & 37.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.037$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-298-B & 05:41:37.040 & -02:17:18.01 & HOPS-298  & 2.2 & None      & -99.0 & 29.4 & 169.3 & I    & 85.83$\pm$4.29 & -99.00$\pm$-99.00  & 0.11$\times$0.11 & 15.4 & 21.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-297   & 05:41:23.294 & -02:17:35.79 & HOPS-297  & 0.3 & HOPS-399  & 40.9 & 0.2 & 274.9 & I    & 3.05$\pm$0.66 & 0.05$\pm$0.05  & 0.19$\times$0.07 & 173.2 & 37.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.034$\pm$0.034 & 1.8 & 0.44\\
HOPS-399   & 05:41:24.932 & -02:18:06.68 & HOPS-399  & 1.8 & HOPS-399  & 1.8 & 6.0 & 31.1 & 0    & 290.39$\pm$6.27 & 0.63$\pm$0.02  & 0.19$\times$0.15 & 143.6 & 38.2 & 0.07$\times$0.07 & 104.3 & 14.0 & 0.059$\pm$0.001 & 0.177$\pm$0.006 & 2.6 & 0.06\\
HOPS-372   & 05:41:26.370 & -02:18:20.18 & HOPS-372  & 0.5 & HOPS-372  & 0.5 & 4.5 & 37.3 & 0    & 20.46$\pm$0.80 & 0.14$\pm$0.02  & 0.10$\times$0.08 & 116.2 & 20.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.043$\pm$0.005 & 2.1 & 0.08\\
HOPS-398   & 05:41:29.414 & -02:21:16.42 & HOPS-398  & 0.7 & HOPS-398  & 0.7 & 1.0 & 23.0 & 0    & 234.84$\pm$5.17 & 0.33$\pm$0.03  & 0.22$\times$0.19 & 10.6 & 44.4 & 0.11$\times$0.08 & 7.4 & 22.4 & 0.082$\pm$0.002 & 0.151$\pm$0.012 & 2.8 & 0.07\\
HOPS-295   & 05:41:28.961 & -02:23:19.56 & HOPS-295  & 0.3 & None      & -99.0 & 0.3 & 86.6 & I    & 3.48$\pm$0.39 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-294   & 05:40:51.733 & -02:26:49.02 & HOPS-294  & 0.5 & None      & -99.0 & 2.6 & 606.8 & Flat & 2.79$\pm$0.49 & -99.00$\pm$-99.00  & 0.11$\times$0.01 & 6.3 & 22.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-107   & 05:35:23.353 & -04:40:10.29 & HOPS-107  & 0.2 & None      & -99.0 & 4.4 & 472.0 & Flat & 37.85$\pm$0.76 & -99.00$\pm$-99.00  & 0.08$\times$0.05 & 120.5 & 16.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.008$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-105   & 05:35:32.299 & -04:46:48.44 & HOPS-105  & 0.2 & None      & -99.0 & 0.1 & 520.3 & Flat & 3.72$\pm$0.84 & -99.00$\pm$-99.00  & 0.14$\times$0.10 & 27.1 & 28.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-102   & 05:34:35.168 & -04:52:17.96 & HOPS-102  & 0.2 & None      & -99.0 & 0.5 & 479.2 & I    & 36.59$\pm$1.48 & -99.00$\pm$-99.00  & 0.47$\times$0.10 & 108.9 & 93.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.015$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
S13-021010 & \nodata & \nodata & S13-021010 & 0.0 & None      & -99.0 & -99.0 & -99.0 & \nodata & 0.72$\pm$0.72 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-100   & \nodata & \nodata & HOPS-100  & 0.0 & None      & -99.0 & 0.0 & 605.1 & I    & 0.63$\pm$0.63 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-99    & 05:34:29.468 & -04:55:30.25 & HOPS-99   & 0.6 & HOPS-99   & 0.6 & 1.2 & 48.9 & 0    & 13.04$\pm$0.65 & 0.09$\pm$0.02  & 0.10$\times$0.07 & 27.3 & 19.2 & 0.06$\times$0.02 & 39.0 & 12.4 & 0.004$\pm$0.000 & 0.035$\pm$0.006 & 2.1 & 0.10\\
HOPS-96    & 05:35:29.718 & -04:58:48.60 & HOPS-96   & 0.2 & HOPS-96   & 0.2 & 5.4 & 35.6 & 0    & 208.90$\pm$3.60 & 0.85$\pm$0.02  & 0.12$\times$0.11 & 134.6 & 24.8 & 0.08$\times$0.07 & 164.1 & 16.4 & 0.040$\pm$0.001 & 0.228$\pm$0.006 & 2.4 & 0.06\\
V2273Ori   & 05:35:15.602 & -04:59:27.96 & None      & -99.0 & HOPS-94   & 35.3 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.14$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.057$\pm$0.005 & -99.0 & -99.00\\
HOPS-383   & 05:35:29.785 & -04:59:50.41 & HOPS-383  & 0.8 & HOPS-383  & 0.8 & 6.8 & 45.8 & 0    & 158.83$\pm$3.12 & 0.46$\pm$0.02  & 0.18$\times$0.12 & 49.7 & 37.0 & 0.06$\times$0.06 & 147.6 & 12.2 & 0.029$\pm$0.001 & 0.117$\pm$0.005 & 2.5 & 0.06\\
HOPS-95    & 05:35:34.205 & -04:59:52.41 & HOPS-95   & 0.2 & HOPS-95   & 0.2 & 0.7 & 41.8 & 0    & 16.14$\pm$0.66 & 0.04$\pm$0.01  & 0.11$\times$0.06 & 36.2 & 21.6 & 0.03$\times$0.00 & 34.3 & 5.4 & 0.006$\pm$0.000 & 0.020$\pm$0.005 & 2.5 & 0.12\\
HOPS-94    & \nodata & \nodata & HOPS-94   & 0.3 & HOPS-94   & 0.3 & 5.7 & 123.0 & I    & 1.00$\pm$1.00 & 0.05$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 49.2 & 6.4 & 0.000$\pm$0.000 & 0.014$\pm$0.002 & 1.2 & 0.44\\
HOPS-93    & 05:35:15.048 & -05:00:08.05 & HOPS-93   & 0.3 & HOPS-94   & 17.5 & 0.4 & 107.3 & I    & 46.99$\pm$1.29 & 0.28$\pm$0.03  & 0.30$\times$0.07 & 121.8 & 59.6 & 0.11$\times$0.07 & 135.8 & 21.4 & 0.020$\pm$0.001 & 0.150$\pm$0.013 & 2.2 & 0.07\\
J05351805-050017.98 & 05:35:18.051 & -05:00:17.98 & HOPS-92   & 15.5 & HOPS-94   & 32.4 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.17$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.04$\times$0.03 & 128.5 & 8.8 & -99.000$\pm$-99.000 & 0.069$\pm$0.004 & -99.0 & -99.00\\
HOPS-92-A-A & 05:35:18.337 & -05:00:32.94 & HOPS-92   & 0.3 & HOPS-91   & 19.9 & 17.6 & 186.3 & Flat & 129.22$\pm$3.27 & 0.32$\pm$0.02  & 0.11$\times$0.10 & 140.8 & 22.8 & 0.07$\times$0.06 & 172.9 & 14.4 & 0.018$\pm$0.000 & 0.063$\pm$0.004 & 2.6 & 0.07\\
HOPS-92-A-B & 05:35:18.328 & -05:00:33.18 & HOPS-92   & 0.3 & HOPS-91   & 19.7 & 17.6 & 186.3 & Flat & 4.36$\pm$1.00 & 0.08$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.02$\times$0.01 & 56.4 & 3.2 & 0.001$\pm$0.000 & 0.015$\pm$0.002 & 1.7 & 0.12\\
HOPS-92-B  & 05:35:18.270 & -05:00:33.92 & HOPS-92   & 1.2 & HOPS-91   & 19.5 & 17.6 & 186.3 & Flat & 171.83$\pm$4.21 & 0.70$\pm$0.02  & 0.17$\times$0.12 & 174.1 & 34.8 & 0.10$\times$0.07 & 150.3 & 19.6 & 0.024$\pm$0.001 & 0.140$\pm$0.004 & 2.4 & 0.06\\
HOPS-91    & 05:35:18.925 & -05:00:51.11 & HOPS-91   & 0.3 & HOPS-91   & 0.3 & 3.6 & 41.7 & 0    & 31.58$\pm$1.57 & 0.02$\pm$0.02  & 0.26$\times$0.20 & 54.4 & 52.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & 0.007$\pm$0.007 & 3.1 & 0.43\\
HOPS-90    & 05:35:34.492 & -05:00:52.34 & HOPS-90   & 0.4 & None      & -99.0 & 2.4 & 417.7 & Flat & 3.93$\pm$0.77 & -99.00$\pm$-99.00  & 0.19$\times$0.11 & 110.4 & 38.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-89    & 05:35:19.975 & -05:01:02.56 & HOPS-89   & 0.3 & HOPS-91   & 19.7 & 1.4 & 158.3 & Flat & 22.90$\pm$0.71 & 0.18$\pm$0.02  & 0.12$\times$0.05 & 82.4 & 23.6 & 0.08$\times$0.04 & 82.3 & 16.0 & 0.007$\pm$0.000 & 0.070$\pm$0.007 & 2.1 & 0.08\\
HOPS-88    & 05:35:22.471 & -05:01:14.31 & HOPS-88   & 0.6 & HOPS-87-88 & 11.7 & 13.8 & 42.4 & 0    & 141.98$\pm$2.46 & 0.70$\pm$0.02  & 0.10$\times$0.09 & 166.9 & 20.4 & 0.06$\times$0.04 & 169.6 & 11.0 & 0.021$\pm$0.000 & 0.148$\pm$0.003 & 2.3 & 0.06\\
HOPS-87    & 05:35:23.420 & -05:01:30.54 & HOPS-87   & 2.0 & HOPS-87-88 & 10.1 & 31.9 & 38.1 & 0    & 1587.40$\pm$33.47 & 2.63$\pm$0.03  & 0.36$\times$0.35 & 11.1 & 72.8 & 0.13$\times$0.11 & 29.7 & 26.0 & 0.188$\pm$0.004 & 0.453$\pm$0.005 & 2.7 & 0.06\\
HOPS-86-A  & 05:35:23.654 & -05:01:40.26 & HOPS-86   & 0.1 & HOPS-87-88 & 19.7 & 2.9 & 112.7 & I    & 25.94$\pm$3.30 & 0.03$\pm$0.03  & 0.17$\times$0.15 & 0.5 & 33.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.001 & 0.009$\pm$0.009 & 2.9 & 0.44\\
HOPS-86-B  & 05:35:23.733 & -05:01:48.13 & HOPS-86   & 8.0 & HOPS-87-88 & 27.0 & 2.9 & 112.7 & I    & 59.35$\pm$2.64 & 0.03$\pm$0.03  & 0.13$\times$0.12 & 7.2 & 25.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.014$\pm$0.001 & 0.009$\pm$0.009 & 3.3 & 0.43\\
HOPS-85-A  & 05:35:28.189 & -05:03:41.20 & HOPS-85   & 0.3 & HOPS-84   & 27.9 & 14.2 & 174.2 & Flat & 29.76$\pm$1.14 & 0.50$\pm$0.03  & 0.05$\times$0.04 & 123.9 & 10.6 & 0.13$\times$0.09 & 146.7 & 26.0 & 0.004$\pm$0.000 & 0.106$\pm$0.006 & 1.7 & 0.07\\
HOPS-85-B  & 05:35:28.193 & -05:03:41.29 & HOPS-85   & 0.4 & HOPS-84   & 27.9 & 14.2 & 174.2 & Flat & 20.90$\pm$0.85 & 0.06$\pm$0.01  & 0.03$\times$0.01 & 66.0 & 5.4 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.003$\pm$0.000 & 0.013$\pm$0.001 & 2.5 & 0.08\\
HOPS-84-A  & 05:35:26.560 & -05:03:55.12 & HOPS-84   & 0.1 & HOPS-84   & 0.1 & 42.9 & 90.8 & I    & 436.20$\pm$8.17 & 1.17$\pm$0.02  & 0.26$\times$0.12 & 167.5 & 52.4 & 0.11$\times$0.06 & 161.3 & 22.0 & 0.048$\pm$0.001 & 0.187$\pm$0.004 & 2.5 & 0.06\\
HOPS-84-B  & 05:35:26.537 & -05:03:55.73 & HOPS-84   & 0.8 & HOPS-84   & 0.8 & 42.9 & 90.8 & I    & 25.09$\pm$3.69 & 0.15$\pm$0.02  & 0.09$\times$0.03 & 166.2 & 18.2 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.003$\pm$0.000 & 0.023$\pm$0.002 & 2.2 & 0.10\\
HOPS-82    & 05:35:19.740 & -05:04:54.50 & HOPS-82   & 0.2 & None      & -99.0 & 2.1 & 116.4 & Flat & 6.16$\pm$0.49 & -99.00$\pm$-99.00  & 0.06$\times$0.04 & 90.9 & 12.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-81    & 05:35:28.019 & -05:04:57.35 & HOPS-81   & 1.3 & HOPS-81   & 1.3 & 1.1 & 40.1 & 0    & 64.33$\pm$1.15 & 0.42$\pm$0.02  & 0.10$\times$0.06 & 122.0 & 19.4 & 0.07$\times$0.03 & 110.1 & 13.0 & 0.020$\pm$0.000 & 0.172$\pm$0.007 & 2.1 & 0.06\\
HOPS-80    & 05:35:25.183 & -05:05:09.37 & HOPS-80   & 0.1 & HOPS-78   & 35.6 & 0.1 & 275.3 & Flat & 14.86$\pm$1.22 & 0.04$\pm$0.04  & 0.27$\times$0.21 & 155.3 & 53.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.001 & 0.030$\pm$0.030 & 2.6 & 0.43\\
HOPS-78-A  & 05:35:25.966 & -05:05:43.33 & HOPS-78   & 2.1 & HOPS-78   & 2.2 & 7.8 & 38.1 & 0    & 322.44$\pm$3.44 & 0.82$\pm$0.02  & 0.44$\times$0.14 & 171.1 & 88.2 & 0.09$\times$0.08 & 49.5 & 18.8 & 0.056$\pm$0.001 & 0.203$\pm$0.005 & 2.6 & 0.06\\
HOPS-78-B  & 05:35:26.148 & -05:05:45.80 & HOPS-78   & 5.3 & HOPS-78   & 5.3 & 7.8 & 38.1 & 0    & 8.53$\pm$1.12 & 0.09$\pm$0.01  & 0.05$\times$0.05 & 179.4 & 10.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.001$\pm$0.000 & 0.022$\pm$0.003 & 2.0 & 0.11\\
HOPS-77-B  & 05:35:31.470 & -05:05:46.10 & HOPS-77   & 1.5 & None      & -99.0 & 11.3 & 550.3 & Flat & 1.42$\pm$0.24 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-78-C  & 05:35:26.181 & -05:05:47.12 & HOPS-78   & 6.4 & HOPS-78   & 6.4 & 7.8 & 38.1 & 0    & 9.34$\pm$1.80 & 0.04$\pm$0.01  & 0.17$\times$0.08 & 131.9 & 33.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.010$\pm$0.002 & 2.3 & 0.12\\
HOPS-77-A-A & 05:35:31.539 & -05:05:47.33 & HOPS-77   & 0.1 & None      & -99.0 & 11.3 & 550.3 & Flat & 6.38$\pm$0.24 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-77-A-B & 05:35:31.545 & -05:05:47.40 & HOPS-77   & 0.2 & None      & -99.0 & 11.3 & 550.3 & Flat & 5.30$\pm$0.24 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-78-D  & 05:35:25.920 & -05:05:47.70 & HOPS-78   & 4.3 & HOPS-78   & 4.3 & 7.8 & 38.1 & 0    & 6.57$\pm$1.48 & 0.02$\pm$0.02  & 0.15$\times$0.03 & 175.4 & 30.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.006$\pm$0.006 & 2.4 & 0.44\\
HOPS-76    & 05:35:25.763 & -05:05:58.13 & HOPS-76   & 0.3 & HOPS-78   & 14.5 & 1.6 & 135.5 & I    & 13.14$\pm$0.47 & 0.21$\pm$0.02  & 0.05$\times$0.04 & 57.6 & 10.8 & 0.14$\times$0.07 & 27.5 & 27.0 & 0.004$\pm$0.000 & 0.076$\pm$0.008 & 1.8 & 0.08\\
HOPS-75-A  & 05:35:26.680 & -05:06:10.51 & HOPS-75   & 0.4 & HOPS-75   & 0.4 & 3.5 & 67.9 & 0    & 16.07$\pm$0.52 & 0.18$\pm$0.02  & 0.06$\times$0.04 & 156.1 & 11.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.054$\pm$0.005 & 1.9 & 0.07\\
HOPS-75-B  & 05:35:26.678 & -05:06:10.76 & HOPS-75   & 0.6 & HOPS-75   & 0.6 & 3.5 & 67.9 & 0    & 1.92$\pm$0.27 & 0.02$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.007$\pm$0.007 & 1.9 & 0.44\\
HOPS-74    & 05:35:24.874 & -05:06:21.58 & HOPS-74   & 0.3 & HOPS-75   & 28.9 & 1.0 & 516.5 & Flat & 42.05$\pm$0.95 & 0.11$\pm$0.01  & 0.12$\times$0.08 & 126.7 & 23.2 & 0.03$\times$0.03 & 29.9 & 5.8 & 0.013$\pm$0.000 & 0.045$\pm$0.004 & 2.5 & 0.07\\
HOPS-73    & 05:35:27.699 & -05:07:04.32 & HOPS-73   & 0.8 & HOPS-73   & 0.8 & 1.5 & 43.0 & 0    & 10.40$\pm$1.14 & 0.06$\pm$0.02  & 0.19$\times$0.16 & 60.9 & 37.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.003$\pm$0.000 & 0.023$\pm$0.006 & 2.2 & 0.14\\
HOPS-72    & 05:35:25.724 & -05:07:46.24 & HOPS-71   & 11.2 & HOPS-394  & 27.8 & 0.5 & 693.0 & \nodata & 16.71$\pm$0.84 & 0.03$\pm$0.03  & 0.11$\times$0.06 & 101.5 & 22.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & 0.015$\pm$0.015 & 2.7 & 0.43\\
HOPS-394-A & 05:35:24.046 & -05:07:52.11 & HOPS-394  & 2.2 & HOPS-394  & 2.3 & 5.7 & 45.5 & 0    & 21.52$\pm$1.38 & 0.24$\pm$0.02  & 0.25$\times$0.13 & 80.7 & 50.0 & 0.12$\times$0.04 & 25.0 & 24.4 & 0.004$\pm$0.000 & 0.063$\pm$0.006 & 1.9 & 0.08\\
HOPS-394-B & 05:35:24.867 & -05:07:54.64 & HOPS-71   & 11.4 & HOPS-394  & 14.1 & 5.7 & 45.5 & 0    & 9.88$\pm$0.32 & 0.06$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.016$\pm$0.002 & 2.2 & 0.08\\
HOPS-71-B  & 05:35:25.541 & -05:07:56.84 & HOPS-71   & 1.1 & HOPS-394  & 24.4 & 4.9 & 277.5 & I    & 5.46$\pm$1.59 & 0.03$\pm$0.03  & 0.29$\times$0.12 & 82.4 & 57.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.009$\pm$0.009 & 2.2 & 0.45\\
HOPS-71-A  & 05:35:25.582 & -05:07:57.64 & HOPS-71   & 0.5 & HOPS-394  & 25.1 & 4.9 & 277.5 & I    & 130.08$\pm$1.12 & 1.11$\pm$0.02  & 0.19$\times$0.07 & 123.0 & 38.0 & 0.08$\times$0.07 & 111.8 & 16.0 & 0.026$\pm$0.000 & 0.306$\pm$0.007 & 2.0 & 0.06\\
HOPS-70-B-B & 05:35:22.570 & -05:08:00.32 & HOPS-70   & 5.1 & HOPS-394  & 21.4 & 6.0 & 619.3 & Flat & 7.89$\pm$0.53 & 0.07$\pm$0.01  & 0.07$\times$0.03 & 51.2 & 13.6 & 0.03$\times$0.01 & 104.4 & 6.0 & 0.001$\pm$0.000 & 0.019$\pm$0.002 & 2.0 & 0.08\\
HOPS-70-B-A & \nodata & \nodata & HOPS-70   & 4.6 & HOPS-394  & 21.6 & 6.0 & 619.3 & Flat & 0.77$\pm$0.77 & 0.13$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.01 & 104.4 & 6.0 & 0.000$\pm$0.000 & 0.033$\pm$0.002 & 0.8 & 0.43\\
HOPS-70-C  & 05:35:21.938 & -05:08:04.58 & HOPS-70   & 7.1 & HOPS-394  & 31.7 & 6.0 & 619.3 & Flat & 8.63$\pm$0.84 & 0.03$\pm$0.03  & 0.17$\times$0.07 & 78.3 & 33.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.009$\pm$0.009 & 2.4 & 0.43\\
HOPS-70-A-B & 05:35:22.426 & -05:08:05.03 & HOPS-70   & 0.3 & HOPS-394  & 25.2 & 6.0 & 619.3 & Flat & 3.37$\pm$0.54 & 0.04$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.03$\times$0.01 & 104.4 & 6.0 & 0.001$\pm$0.000 & 0.010$\pm$0.002 & 1.9 & 0.13\\
HOPS-70-A-A & 05:35:22.406 & -05:08:05.14 & HOPS-70   & 0.4 & HOPS-394  & 25.5 & 6.0 & 619.3 & Flat & 35.89$\pm$0.54 & 0.29$\pm$0.02  & 0.05$\times$0.05 & 13.4 & 10.4 & 0.05$\times$0.04 & 72.2 & 9.8 & 0.007$\pm$0.000 & 0.076$\pm$0.004 & 2.1 & 0.07\\
HOPS-350   & \nodata & \nodata & HOPS-350  & 0.0 & HOPS-350  & 0.0 & 0.5 & 57.3 & I    & 0.70$\pm$0.70 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.013$\pm$0.013 & 1.4 & 0.61\\
HOPS-68    & 05:35:24.299 & -05:08:30.74 & HOPS-68   & 0.2 & HOPS-68   & 0.0 & 5.0 & 100.6 & I    & 88.22$\pm$1.59 & 0.44$\pm$0.02  & 0.10$\times$0.09 & 3.6 & 19.2 & 0.04$\times$0.04 & 150.8 & 9.0 & 0.018$\pm$0.000 & 0.121$\pm$0.004 & 2.3 & 0.06\\
HOPS-66-B  & 05:35:26.927 & -05:09:22.43 & HOPS-66   & 2.5 & HOPS-370  & 15.2 & 18.3 & 264.9 & Flat & 34.62$\pm$1.10 & 0.08$\pm$0.01  & 0.17$\times$0.12 & 165.8 & 34.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.005$\pm$0.000 & 0.015$\pm$0.003 & 2.6 & 0.09\\
HOPS-66-A  & 05:35:26.857 & -05:09:24.40 & HOPS-66   & 0.3 & HOPS-370  & 14.7 & 18.3 & 264.9 & Flat & 43.31$\pm$0.57 & 0.29$\pm$0.01  & 0.05$\times$0.04 & 47.0 & 10.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.006$\pm$0.000 & 0.058$\pm$0.003 & 2.1 & 0.06\\
HOPS-370   & 05:35:27.634 & -05:09:34.42 & HOPS-370  & 1.0 & HOPS-370  & 1.0 & 315.7 & 71.5 & I    & 533.28$\pm$10.05 & 2.84$\pm$0.02  & 0.34$\times$0.11 & 109.7 & 67.6 & 0.08$\times$0.03 & 5.6 & 16.8 & 0.034$\pm$0.001 & 0.275$\pm$0.002 & 2.2 & 0.06\\
HOPS-65    & 05:35:21.576 & -05:09:38.85 & HOPS-65   & 0.4 & None      & -99.0 & 0.3 & 545.7 & I    & 83.91$\pm$3.20 & -99.00$\pm$-99.00  & 0.99$\times$0.28 & 171.4 & 198.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.038$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
2MJ05352746-0509441 & 05:35:27.472 & -05:09:44.14 & HOPS-370  & 10.9 & HOPS-370  & 10.9 & -99.0 & -99.0 & II   & 9.07$\pm$1.79 & 0.15$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.09$\times$0.03 & 10.9 & 18.8 & 0.003$\pm$0.001 & 0.060$\pm$0.007 & 1.8 & 0.12\\
HOPS-64    & 05:35:26.998 & -05:09:54.08 & HOPS-108  & 6.4 & HOPS-108  & 6.4 & 13.4 & 29.7 & I    & 33.47$\pm$0.76 & 0.26$\pm$0.02  & 0.10$\times$0.07 & 119.3 & 19.0 & 0.06$\times$0.05 & 158.6 & 11.8 & 0.005$\pm$0.000 & 0.055$\pm$0.004 & 2.1 & 0.07\\
HOPS-108   & 05:35:27.086 & -05:10:00.06 & HOPS-108  & 0.4 & HOPS-108  & 0.4 & 33.5 & 38.5 & 0    & 62.63$\pm$0.98 & 0.10$\pm$0.02  & 0.12$\times$0.12 & 105.7 & 24.2 & 0.07$\times$0.06 & 156.2 & 14.2 & 0.007$\pm$0.000 & 0.017$\pm$0.003 & 2.8 & 0.10\\
VLA16      & 05:35:26.824 & -05:10:05.62 & HOPS-108  & 6.4 & HOPS-108  & 6.4 & -99.0 & -99.0 & \nodata & 6.66$\pm$0.81 & 0.04$\pm$0.01  & 0.10$\times$0.08 & 164.8 & 19.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.017$\pm$0.005 & 2.2 & 0.15\\
VLA15      & 05:35:26.410 & -05:10:05.94 & HOPS-108  & 11.4 & HOPS-108  & 11.4 & -99.0 & -99.0 & \nodata & 122.94$\pm$1.65 & 0.53$\pm$0.03  & 0.41$\times$0.11 & 87.3 & 81.6 & 0.18$\times$0.07 & 85.7 & 35.2 & 0.039$\pm$0.001 & 0.220$\pm$0.013 & 2.3 & 0.07\\
OMC2-FIR4-ALMA1 & 05:35:26.785 & -05:10:08.83 & HOPS-369  & 8.8 & HOPS-108  & 9.5 & -99.0 & -99.0 & \nodata & 5.57$\pm$0.73 & 0.06$\pm$0.01  & 0.14$\times$0.04 & 110.5 & 29.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.024$\pm$0.005 & 1.9 & 0.13\\
HOPS-369   & 05:35:26.969 & -05:10:17.27 & HOPS-369  & 0.1 & HOPS-108  & 17.0 & 30.9 & 379.2 & Flat & 26.11$\pm$0.53 & 0.05$\pm$0.01  & 0.05$\times$0.04 & 21.3 & 9.4 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.003$\pm$0.000 & 0.009$\pm$0.001 & 2.7 & 0.08\\
HOPS-368   & 05:35:24.725 & -05:10:30.08 & HOPS-368  & 0.1 & HOPS-108  & 46.0 & 60.2 & 137.5 & I    & 135.91$\pm$2.62 & 1.10$\pm$0.02  & 0.19$\times$0.08 & 105.2 & 37.2 & 0.06$\times$0.03 & 72.6 & 11.4 & 0.014$\pm$0.000 & 0.162$\pm$0.003 & 2.1 & 0.06\\
HOPS-60    & 05:35:23.287 & -05:12:03.41 & HOPS-60   & 0.7 & HOPS-60   & 0.7 & 19.2 & 54.1 & 0    & 336.12$\pm$5.98 & 1.21$\pm$0.02  & 0.19$\times$0.11 & 159.0 & 37.6 & 0.08$\times$0.06 & 153.5 & 16.8 & 0.046$\pm$0.001 & 0.237$\pm$0.004 & 2.4 & 0.06\\
2MJ05352131-0512126 & 05:35:21.318 & -05:12:12.68 & None      & -99.0 & HOPS-60   & 31.5 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.28$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.10$\times$0.04 & 77.2 & 19.8 & -99.000$\pm$-99.000 & 0.117$\pm$0.010 & -99.0 & -99.00\\
HOPS-59-B  & 05:35:20.134 & -05:13:13.31 & HOPS-59   & 2.2 & HOPS-409  & 19.4 & 43.2 & 528.4 & Flat & 7.25$\pm$1.93 & 0.08$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.001$\pm$0.000 & 0.013$\pm$0.001 & 1.9 & 0.14\\
HOPS-59-A  & 05:35:20.151 & -05:13:15.70 & HOPS-59   & 0.2 & HOPS-409  & 18.7 & 43.2 & 528.4 & Flat & 309.07$\pm$6.00 & 1.48$\pm$0.04  & 0.25$\times$0.16 & 91.8 & 50.6 & 0.14$\times$0.10 & 91.6 & 28.0 & 0.034$\pm$0.001 & 0.236$\pm$0.007 & 2.3 & 0.06\\
HOPS-409   & 05:35:21.363 & -05:13:17.83 & HOPS-409  & 0.6 & HOPS-409  & 0.6 & 7.2 & 28.4 & 0    & 185.41$\pm$1.90 & 0.82$\pm$0.04  & 0.34$\times$0.12 & 115.8 & 67.2 & 0.16$\times$0.06 & 108.5 & 32.8 & 0.033$\pm$0.000 & 0.205$\pm$0.009 & 2.3 & 0.06\\
HOPS-58    & 05:35:18.523 & -05:13:38.34 & HOPS-58   & 0.3 & HOPS-409  & 47.8 & 3.9 & 620.0 & Flat & 111.07$\pm$2.23 & 0.14$\pm$0.01  & 0.16$\times$0.14 & 172.4 & 31.2 & 0.03$\times$0.02 & 75.1 & 5.0 & 0.024$\pm$0.000 & 0.042$\pm$0.003 & 2.8 & 0.07\\
HOPS-57-A  & 05:35:19.887 & -05:15:08.18 & HOPS-57   & 0.8 & HOPS-56   & 25.3 & 2.8 & 421.2 & Flat & 131.13$\pm$2.62 & 0.53$\pm$0.02  & 0.23$\times$0.12 & 43.0 & 45.2 & 0.07$\times$0.04 & 13.1 & 13.4 & 0.031$\pm$0.001 & 0.169$\pm$0.006 & 2.4 & 0.06\\
HOPS-57-B  & 05:35:19.833 & -05:15:09.03 & HOPS-57   & 0.5 & HOPS-56   & 24.3 & 2.8 & 421.2 & Flat & 10.96$\pm$1.17 & 0.03$\pm$0.03  & 0.06$\times$0.03 & 74.0 & 12.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & 0.008$\pm$0.008 & 2.6 & 0.43\\
HOPS-56-A-C & 05:35:19.481 & -05:15:32.81 & HOPS-56   & 0.3 & HOPS-56   & 0.2 & 20.4 & 48.1 & 0    & 2.77$\pm$0.26 & 0.03$\pm$0.03  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.005$\pm$0.005 & 2.0 & 0.43\\
HOPS-56-D  & 05:35:17.922 & -05:15:32.84 & None      & -99.0 & HOPS-56   & 23.1 & 20.4 & 48.1 & 0    & -99.00$\pm$-99.00 & 0.14$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.10$\times$0.06 & 116.4 & 20.6 & -99.000$\pm$-99.000 & 0.026$\pm$0.005 & -99.0 & -99.00\\
V1334Ori   & 05:35:17.923 & -05:15:32.84 & None      & -99.0 & HOPS-56   & 23.0 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.14$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.13$\times$0.06 & 119.2 & 26.2 & -99.000$\pm$-99.000 & 0.060$\pm$0.011 & -99.0 & -99.00\\
HOPS-56-A-B & 05:35:19.470 & -05:15:32.96 & HOPS-56   & 0.3 & HOPS-56   & 0.3 & 20.4 & 48.1 & 0    & 2.32$\pm$0.26 & 0.08$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.000$\pm$0.000 & 0.015$\pm$0.003 & 1.4 & 0.12\\
HOPS-56-A-A & 05:35:19.482 & -05:15:33.08 & HOPS-56   & 0.4 & HOPS-56   & 0.4 & 20.4 & 48.1 & 0    & 12.08$\pm$0.58 & 0.14$\pm$0.02  & 0.07$\times$0.05 & 43.2 & 13.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.026$\pm$0.003 & 1.9 & 0.08\\
V2358Ori   & 05:35:19.811 & -05:15:35.20 & HOPS-56   & 5.7 & HOPS-56   & 5.7 & -99.0 & -99.0 & \nodata & 2.72$\pm$0.54 & 0.07$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.09$\times$0.01 & 138.8 & 17.6 & 0.001$\pm$0.000 & 0.031$\pm$0.008 & 1.5 & 0.15\\
HOPS-56-B  & 05:35:19.420 & -05:15:38.29 & HOPS-56   & 5.6 & HOPS-56   & 5.6 & 20.4 & 48.1 & 0    & 129.68$\pm$3.77 & 0.15$\pm$0.03  & 0.79$\times$0.39 & 61.1 & 158.6 & 0.20$\times$0.03 & 133.7 & 39.2 & 0.017$\pm$0.001 & 0.029$\pm$0.005 & 2.9 & 0.10\\
J05352074-0515492 & 05:35:20.751 & -05:15:49.26 & None      & -99.0 & HOPS-56   & 25.3 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 1.13$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 139.7 & 6.0 & -99.000$\pm$-99.000 & 0.467$\pm$0.007 & -99.0 & -99.00\\
OMC1N-1-A  & 05:35:17.890 & -05:18:35.41 & None      & -99.0 & OMC1N-1   & 9.8 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.05$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 5.7 & 6.0 & -99.000$\pm$-99.000 & 0.021$\pm$0.004 & -99.0 & -99.00\\
OMC1N-1-B  & 05:35:16.812 & -05:19:01.00 & None      & -99.0 & OMC1N-2-3 & 20.8 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.07$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 5.7 & 6.0 & -99.000$\pm$-99.000 & 0.029$\pm$0.004 & -99.0 & -99.00\\
OMC1N-1-C  & 05:35:17.145 & -05:19:12.70 & None      & -99.0 & OMC1N-2-3 & 8.9 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.09$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 5.7 & 6.0 & -99.000$\pm$-99.000 & 0.036$\pm$0.004 & -99.0 & -99.00\\
OMC1N-2-3  & 05:35:16.611 & -05:19:35.69 & None      & -99.0 & OMC1N-2-3 & 15.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.07$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.03$\times$0.02 & 6.3 & 6.2 & -99.000$\pm$-99.000 & 0.031$\pm$0.004 & -99.0 & -99.00\\
OMC1N-4-5-A & 05:35:16.040 & -05:19:44.61 & None      & -99.0 & OMC1N-4-5 & 24.0 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.69$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.284$\pm$0.006 & -99.0 & -99.00\\
OMC1N-4-5-B & 05:35:16.047 & -05:20:05.61 & None      & -99.0 & OMC1N-4-5 & 3.1 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.09$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.036$\pm$0.002 & -99.0 & -99.00\\
OMC1N-4-5-C & 05:35:15.973 & -05:20:14.25 & None      & -99.0 & OMC1N-4-5 & 5.6 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.59$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.07$\times$0.05 & 148.9 & 14.6 & -99.000$\pm$-99.000 & 0.243$\pm$0.008 & -99.0 & -99.00\\
OMC1N-6-7-8-A-A & 05:35:18.673 & -05:20:33.71 & None      & -99.0 & OMC1N-6-7-8 & 30.5 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.88$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.09$\times$0.01 & 67.9 & 17.6 & -99.000$\pm$-99.000 & 0.362$\pm$0.008 & -99.0 & -99.00\\
OMC1N-6-7-8-A-B & 05:35:18.660 & -05:20:33.82 & None      & -99.0 & OMC1N-6-7-8 & 30.3 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.08$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.032$\pm$0.002 & -99.0 & -99.00\\
OMC1N-6-7-8-E & 05:35:15.698 & -05:20:39.32 & None      & -99.0 & OMC1N-6-7-8 & 15.4 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.53$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.05$\times$0.03 & 104.2 & 9.2 & -99.000$\pm$-99.000 & 0.221$\pm$0.007 & -99.0 & -99.00\\
OMC1N-6-7-8-D & 05:35:16.659 & -05:20:44.44 & None      & -99.0 & OMC1N-6-7-8 & 2.4 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.30$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.04$\times$0.02 & 43.8 & 7.0 & -99.000$\pm$-99.000 & 0.126$\pm$0.006 & -99.0 & -99.00\\
OMC1N-6-7-8-B & 05:35:18.192 & -05:20:48.46 & None      & -99.0 & OMC1N-6-7-8 & 23.0 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.61$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.09$\times$0.06 & 105.4 & 17.0 & -99.000$\pm$-99.000 & 0.252$\pm$0.010 & -99.0 & -99.00\\
OMC1N-6-7-8-C & 05:35:18.001 & -05:20:55.76 & None      & -99.0 & OMC1N-6-7-8 & 23.6 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.63$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.09$\times$0.07 & 134.5 & 18.4 & -99.000$\pm$-99.000 & 0.262$\pm$0.010 & -99.0 & -99.00\\
OMC1N-6-7-8-F & 05:35:16.278 & -05:21:09.13 & None      & -99.0 & OMC1N-6-7-8 & 27.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.09$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.035$\pm$0.002 & -99.0 & -99.00\\
OMC1N-6-7-8-G & 05:35:15.402 & -05:21:13.98 & None      & -99.0 & OMC1N-6-7-8 & 37.3 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.12$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.050$\pm$0.002 & -99.0 & -99.00\\
OMC1N-6-7-8-H & 05:35:15.604 & -05:21:26.88 & None      & -99.0 & OMC1N-6-7-8 & 47.7 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.25$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.103$\pm$0.002 & -99.0 & -99.00\\
HOPS-53    & 05:33:57.395 & -05:23:29.99 & HOPS-53   & 0.5 & HOPS-53   & 0.5 & 22.8 & 45.9 & 0    & 78.13$\pm$1.25 & 0.63$\pm$0.02  & 0.07$\times$0.05 & 128.7 & 13.0 & 0.05$\times$0.04 & 121.5 & 10.2 & 0.010$\pm$0.000 & 0.116$\pm$0.003 & 2.1 & 0.06\\
HOPS-50    & 05:34:40.914 & -05:31:44.71 & HOPS-50   & 0.3 & HOPS-50   & 0.3 & 3.6 & 51.4 & 0    & 240.58$\pm$4.62 & 0.95$\pm$0.02  & 0.25$\times$0.13 & 68.3 & 49.8 & 0.08$\times$0.06 & 72.1 & 16.4 & 0.052$\pm$0.001 & 0.280$\pm$0.007 & 2.4 & 0.06\\
HOPS-49    & 05:34:48.885 & -05:31:45.79 & HOPS-49   & 0.2 & None      & -99.0 & 0.6 & 356.8 & I    & 13.13$\pm$0.72 & -99.00$\pm$-99.00  & 0.17$\times$0.04 & 27.1 & 34.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-47    & 05:33:45.882 & -05:32:58.12 & HOPS-47   & 0.2 & None      & -99.0 & 0.1 & 558.4 & Flat & 6.08$\pm$0.79 & -99.00$\pm$-99.00  & 0.21$\times$0.11 & 158.5 & 41.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-45-A  & 05:35:06.457 & -05:33:34.98 & HOPS-45   & 0.1 & None      & -99.0 & 7.4 & 517.8 & Flat & 39.09$\pm$0.84 & -99.00$\pm$-99.00  & 0.08$\times$0.04 & 29.0 & 16.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-45-B  & 05:35:06.454 & -05:33:35.28 & HOPS-45   & 0.2 & None      & -99.0 & 7.4 & 517.8 & Flat & 22.57$\pm$0.76 & -99.00$\pm$-99.00  & 0.05$\times$0.04 & 146.8 & 10.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-44    & 05:35:10.591 & -05:35:06.26 & HOPS-44   & 0.3 & HOPS-44   & 0.3 & 1.5 & 43.8 & 0    & 3.48$\pm$0.70 & 0.03$\pm$0.03  & 0.15$\times$0.10 & 101.5 & 29.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.011$\pm$0.011 & 2.0 & 0.44\\
HOPS-43    & 05:35:04.503 & -05:35:14.78 & HOPS-43   & 0.4 & HOPS-43   & 0.4 & 2.8 & 75.0 & I    & 4.59$\pm$0.69 & 0.24$\pm$0.02  & 0.17$\times$0.10 & 120.2 & 34.8 & 0.05$\times$0.03 & 171.2 & 10.6 & 0.001$\pm$0.000 & 0.077$\pm$0.005 & 1.3 & 0.09\\
HOPS-42    & 05:35:05.061 & -05:35:40.79 & HOPS-42   & 0.3 & HOPS-43   & 27.7 & 0.2 & 200.9 & I    & 48.73$\pm$1.51 & 0.02$\pm$0.02  & 0.40$\times$0.10 & 106.2 & 80.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.024$\pm$0.001 & 0.013$\pm$0.013 & 3.3 & 0.43\\
HOPS-41    & 05:34:29.463 & -05:35:42.80 & HOPS-41   & 0.4 & None      & -99.0 & 1.7 & 82.3 & I    & 25.98$\pm$0.56 & -99.00$\pm$-99.00  & 0.04$\times$0.03 & 45.5 & 8.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-40    & 05:35:08.440 & -05:35:58.57 & HOPS-40   & 1.4 & HOPS-40   & 1.4 & 2.3 & 38.1 & 0    & 8.14$\pm$0.69 & 0.10$\pm$0.02  & 0.14$\times$0.07 & 76.1 & 29.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.032$\pm$0.006 & 1.9 & 0.11\\
HOPS-38    & \nodata & \nodata & HOPS-38   & 0.0 & None      & -99.0 & 0.2 & 58.5 & 0    & 0.65$\pm$0.65 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.017$\pm$0.017 & -99.0 & -99.00\\
HOPS-36    & 05:34:26.453 & -05:37:40.75 & HOPS-36   & 0.4 & None      & -99.0 & 0.9 & 374.6 & Flat & 40.16$\pm$0.95 & -99.00$\pm$-99.00  & 0.13$\times$0.07 & 155.4 & 26.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-382   & \nodata & \nodata & HOPS-382  & 0.0 & None      & -99.0 & 0.1 & 204.4 & I    & 0.70$\pm$0.70 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-33    & \nodata & \nodata & HOPS-33   & 0.0 & None      & -99.0 & 0.1 & 777.6 & Flat & 0.64$\pm$0.64 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-32-A  & 05:34:35.454 & -05:39:59.33 & HOPS-32   & 0.2 & HOPS-32   & 0.2 & 1.7 & 58.9 & 0    & 22.20$\pm$0.72 & 0.11$\pm$0.02  & 0.11$\times$0.06 & 52.5 & 21.2 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.006$\pm$0.000 & 0.038$\pm$0.006 & 2.3 & 0.10\\
HOPS-32-B  & 05:34:35.432 & -05:39:59.58 & HOPS-32   & 0.6 & HOPS-32   & 0.5 & 1.7 & 58.9 & 0    & 13.97$\pm$1.01 & 0.12$\pm$0.03  & 0.15$\times$0.11 & 68.5 & 30.8 & 0.17$\times$0.04 & 163.5 & 35.0 & 0.004$\pm$0.000 & 0.044$\pm$0.009 & 2.0 & 0.11\\
HOPS-30    & 05:34:44.055 & -05:41:25.84 & HOPS-30   & 0.1 & None      & -99.0 & 3.3 & 81.2 & I    & 115.09$\pm$2.02 & 0.22$\pm$0.01  & 0.13$\times$0.08 & 139.9 & 25.2 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.025$\pm$0.000 & 0.066$\pm$0.002 & -99.0 & -99.00\\
HOPS-29    & 05:34:49.043 & -05:41:42.40 & HOPS-29   & 0.2 & HOPS-28   & 29.4 & 1.7 & 148.2 & I    & 28.58$\pm$0.67 & 0.14$\pm$0.01  & 0.07$\times$0.06 & 172.5 & 13.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.008$\pm$0.000 & 0.052$\pm$0.003 & 2.3 & 0.06\\
HOPS-28-A  & 05:34:47.320 & -05:41:56.08 & HOPS-28   & 0.5 & HOPS-28   & 0.5 & 0.4 & 46.3 & 0    & 10.08$\pm$0.73 & 0.03$\pm$0.01  & 0.16$\times$0.06 & 54.0 & 31.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.004$\pm$0.000 & 0.013$\pm$0.004 & 2.6 & 0.13\\
HOPS-28-B  & 05:34:47.303 & -05:41:56.29 & HOPS-28   & 0.5 & HOPS-28   & 0.5 & 0.4 & 46.3 & 0    & 2.62$\pm$0.48 & 0.02$\pm$0.02  & 0.08$\times$0.01 & 67.3 & 15.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.011$\pm$0.011 & 2.1 & 0.44\\
HOPS-24    & \nodata & \nodata & HOPS-24   & 0.0 & None      & -99.0 & 0.1 & 288.9 & I    & 0.62$\pm$0.62 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-20-B  & \nodata & \nodata & HOPS-20   & 0.2 & HOPS-20   & 0.2 & 1.1 & 94.8 & I    & 0.70$\pm$0.70 & 0.02$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.000$\pm$0.000 & 0.009$\pm$0.003 & 1.5 & 0.45\\
HOPS-20-A  & 05:33:30.704 & -05:50:41.29 & HOPS-20   & 0.3 & HOPS-20   & 0.3 & 1.1 & 94.8 & I    & 6.71$\pm$0.46 & 0.07$\pm$0.01  & 0.05$\times$0.03 & 59.5 & 10.4 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.028$\pm$0.003 & 2.0 & 0.08\\
HOPS-19    & \nodata & \nodata & HOPS-19   & 0.0 & None      & -99.0 & 0.2 & 101.6 & Flat & 0.63$\pm$0.63 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-18    & 05:35:05.515 & -05:51:54.42 & HOPS-18   & 0.4 & HOPS-18   & 0.4 & 1.2 & 71.8 & I    & 35.09$\pm$1.33 & 0.22$\pm$0.02  & 0.27$\times$0.07 & 161.4 & 54.0 & 0.09$\times$0.07 & 86.9 & 17.4 & 0.010$\pm$0.000 & 0.085$\pm$0.009 & 2.2 & 0.08\\
HOPS-17    & 05:35:07.185 & -05:52:06.07 & HOPS-17   & 0.2 & HOPS-18   & 27.9 & 0.3 & 341.3 & I    & 43.93$\pm$1.13 & 0.07$\pm$0.01  & 0.17$\times$0.10 & 37.2 & 35.0 & 0.01$\times$0.01 & 28.5 & 1.4 & 0.021$\pm$0.001 & 0.039$\pm$0.004 & 2.8 & 0.08\\
HOPS-15    & 05:36:19.027 & -05:55:25.40 & HOPS-15   & 0.1 & None      & -99.0 & 0.1 & 342.0 & Flat & 4.58$\pm$0.60 & -99.00$\pm$-99.00  & 0.11$\times$0.06 & 58.7 & 21.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-16    & 05:35:00.822 & -05:55:26.07 & HOPS-16   & 0.4 & None      & -99.0 & 0.6 & 361.0 & Flat & 21.64$\pm$0.67 & -99.00$\pm$-99.00  & 0.05$\times$0.03 & 147.6 & 9.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.008$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-13    & 05:35:24.581 & -05:55:33.74 & HOPS-13   & 0.5 & None      & -99.0 & 1.0 & 383.6 & Flat & 3.90$\pm$0.70 & -99.00$\pm$-99.00  & 0.19$\times$0.09 & 30.7 & 37.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-371   & 05:35:10.419 & -05:55:40.55 & HOPS-371  & 0.3 & HOPS-12   & 30.4 & 0.5 & 31.6 & 0    & 3.66$\pm$0.69 & 0.03$\pm$0.03  & 0.13$\times$0.10 & 113.4 & 26.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.016$\pm$0.016 & 2.0 & 0.44\\
HOPS-12-A  & 05:35:08.631 & -05:55:54.64 & HOPS-12   & 0.6 & HOPS-12   & 0.6 & 6.3 & 42.0 & 0    & 33.16$\pm$0.73 & 0.17$\pm$0.01  & 0.06$\times$0.05 & 103.3 & 12.4 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.006$\pm$0.000 & 0.043$\pm$0.003 & 2.3 & 0.07\\
HOPS-12-B-B & 05:35:08.955 & -05:55:54.88 & HOPS-12   & 5.3 & HOPS-12   & 5.3 & 6.3 & 42.0 & 0    & 42.34$\pm$0.82 & 0.46$\pm$0.02  & 0.09$\times$0.06 & 82.5 & 17.0 & 0.05$\times$0.03 & 66.6 & 10.8 & 0.008$\pm$0.000 & 0.116$\pm$0.004 & 1.9 & 0.06\\
HOPS-12-B-A & 05:35:08.945 & -05:55:55.03 & HOPS-12   & 5.2 & HOPS-12   & 5.2 & 6.3 & 42.0 & 0    & 59.90$\pm$0.88 & 0.47$\pm$0.02  & 0.09$\times$0.07 & 76.6 & 18.6 & 0.05$\times$0.05 & 148.7 & 10.8 & 0.011$\pm$0.000 & 0.121$\pm$0.004 & 2.1 & 0.06\\
S13-006006 & \nodata & \nodata & S13-006006 & 0.0 & None      & -99.0 & -99.0 & -99.0 & \nodata & 0.72$\pm$0.72 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-11    & 05:35:13.424 & -05:57:57.88 & HOPS-11   & 0.3 & HOPS-11   & 0.3 & 7.7 & 48.8 & 0    & 236.58$\pm$4.14 & 0.40$\pm$0.03  & 0.13$\times$0.12 & 94.4 & 25.4 & 0.10$\times$0.08 & 83.1 & 20.2 & 0.041$\pm$0.001 & 0.097$\pm$0.006 & 2.7 & 0.07\\
HOPS-10    & 05:35:09.050 & -05:58:26.87 & HOPS-10   & 1.0 & HOPS-10   & 1.0 & 2.8 & 46.2 & 0    & 69.21$\pm$1.33 & 0.49$\pm$0.02  & 0.14$\times$0.07 & 116.6 & 28.4 & 0.08$\times$0.05 & 124.8 & 16.0 & 0.016$\pm$0.000 & 0.151$\pm$0.007 & 2.1 & 0.06\\
HOPS-192   & 05:36:32.472 & -06:01:16.45 & HOPS-192  & 0.4 & None      & -99.0 & 1.2 & 202.5 & Flat & 36.03$\pm$1.02 & -99.00$\pm$-99.00  & 0.11$\times$0.09 & 31.5 & 22.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-193-A & 05:36:30.282 & -06:01:17.11 & HOPS-193  & 0.3 & None      & -99.0 & 1.0 & 226.7 & I    & 8.81$\pm$0.53 & -99.00$\pm$-99.00  & 0.05$\times$0.04 & 16.5 & 10.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-193-B & 05:36:30.283 & -06:01:17.37 & HOPS-193  & 0.2 & None      & -99.0 & 1.0 & 226.7 & I    & 8.68$\pm$0.52 & -99.00$\pm$-99.00  & 0.05$\times$0.02 & 149.1 & 10.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-200   & 05:35:33.214 & -06:06:09.62 & HOPS-200  & 0.0 & None      & -99.0 & 0.2 & 244.4 & Flat & 73.37$\pm$2.27 & -99.00$\pm$-99.00  & 0.46$\times$0.16 & 84.1 & 91.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.035$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-194   & 05:35:52.027 & -06:10:01.67 & HOPS-194  & 0.4 & None      & -99.0 & 10.8 & 645.0 & Flat & 270.49$\pm$5.46 & -99.00$\pm$-99.00  & 0.19$\times$0.17 & 86.5 & 38.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.042$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-191   & 05:36:17.273 & -06:11:11.21 & HOPS-191  & 0.3 & None      & -99.0 & 0.5 & 196.7 & I    & 7.93$\pm$0.49 & -99.00$\pm$-99.00  & 0.05$\times$0.02 & 139.2 & 9.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-198   & 05:35:22.196 & -06:13:06.14 & HOPS-198  & 0.3 & HOPS-198  & 0.3 & 0.7 & 61.4 & 0    & 56.26$\pm$1.64 & 0.22$\pm$0.00  & 0.41$\times$0.07 & 158.4 & 81.8 & 0.19$\times$0.13 & 156.2 & 37.2 & 0.019$\pm$0.001 & 0.094$\pm$0.000 & 2.4 & 0.06\\
HOPS-185   & 05:36:36.969 & -06:14:58.78 & HOPS-185  & 0.8 & None      & -99.0 & 0.9 & 96.9 & I    & 21.56$\pm$1.13 & -99.00$\pm$-99.00  & 0.27$\times$0.10 & 94.9 & 54.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-181-B & 05:36:19.655 & -06:22:08.95 & HOPS-181  & 4.1 & HOPS-182  & 12.3 & 5.2 & 131.3 & I    & 19.23$\pm$1.45 & 0.02$\pm$0.02  & 0.11$\times$0.08 & 139.7 & 22.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & 0.006$\pm$0.006 & 2.9 & 0.43\\
HOPS-182-A & 05:36:18.795 & -06:22:10.21 & HOPS-182  & 0.6 & HOPS-182  & 0.5 & 59.8 & 51.9 & 0    & 741.93$\pm$7.97 & 0.72$\pm$0.03  & 0.21$\times$0.16 & 150.8 & 42.6 & 0.12$\times$0.09 & 10.2 & 23.4 & 0.071$\pm$0.001 & 0.102$\pm$0.004 & 3.0 & 0.06\\
HOPS-182-B & 05:36:18.775 & -06:22:11.15 & HOPS-182  & 1.3 & HOPS-182  & 1.3 & 59.8 & 51.9 & 0    & 111.17$\pm$4.08 & 1.22$\pm$0.02  & 0.11$\times$0.06 & 79.4 & 22.2 & 0.06$\times$0.05 & 86.4 & 12.4 & 0.011$\pm$0.000 & 0.173$\pm$0.003 & 1.9 & 0.06\\
HOPS-181-A & 05:36:19.504 & -06:22:11.99 & HOPS-181  & 0.4 & HOPS-182  & 10.2 & 5.2 & 131.3 & I    & 8.42$\pm$0.95 & 0.32$\pm$0.02  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.04$\times$0.04 & 87.4 & 8.6 & 0.002$\pm$0.000 & 0.085$\pm$0.004 & 1.4 & 0.08\\
HOPS-182-C & 05:36:18.478 & -06:22:13.62 & HOPS-182  & 6.3 & HOPS-182  & 6.3 & 59.8 & 51.9 & 0    & 17.03$\pm$3.44 & 0.17$\pm$0.02  & 0.07$\times$0.04 & 127.1 & 13.0 & 0.06$\times$0.03 & 162.1 & 11.0 & 0.002$\pm$0.000 & 0.024$\pm$0.002 & 2.0 & 0.11\\
HOPS-183-B & 05:36:17.912 & -06:22:27.25 & HOPS-183  & 1.1 & HOPS-182  & 21.9 & 0.2 & 224.5 & Flat & 2.10$\pm$0.53 & 0.03$\pm$0.03  & 0.09$\times$0.03 & 117.6 & 17.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.018$\pm$0.018 & 1.8 & 0.45\\
HOPS-183-A & \nodata & \nodata & HOPS-183  & 0.3 & HOPS-182  & 22.7 & 0.2 & 224.5 & Flat & 0.74$\pm$0.74 & 0.22$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.07$\times$0.02 & 30.0 & 13.6 & 0.000$\pm$0.000 & 0.126$\pm$0.009 & 0.5 & 0.43\\
HOPS-178   & 05:36:24.622 & -06:22:41.14 & HOPS-178  & 0.3 & None      & -99.0 & 16.8 & 155.1 & I    & 43.69$\pm$0.93 & -99.00$\pm$-99.00  & 0.10$\times$0.05 & 60.4 & 21.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-187   & \nodata & \nodata & HOPS-187  & 0.0 & None      & -99.0 & 0.2 & 1210.9 & Flat & 0.60$\pm$0.60 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-179   & 05:36:21.876 & -06:23:29.91 & HOPS-179  & 0.6 & None      & -99.0 & 1.6 & 467.5 & Flat & 97.47$\pm$1.95 & -99.00$\pm$-99.00  & 0.13$\times$0.12 & 56.0 & 26.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.026$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-176   & 05:36:23.603 & -06:24:51.48 & HOPS-176  & 0.3 & HOPS-173-380 & 31.5 & 1.3 & 312.2 & Flat & 1.96$\pm$0.75 & 0.20$\pm$0.02  & 0.18$\times$0.09 & 148.5 & 36.4 & 0.06$\times$0.05 & 160.7 & 12.8 & 0.001$\pm$0.000 & 0.074$\pm$0.008 & 1.0 & 0.18\\
HOPS-175   & \nodata & \nodata & HOPS-175  & 0.0 & HOPS-173-380 & 23.9 & 0.3 & 104.3 & I    & 0.63$\pm$0.63 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.016$\pm$0.016 & 1.3 & 0.61\\
HOPS-174   & 05:36:25.868 & -06:24:58.67 & HOPS-174  & 0.2 & HOPS-173-380 & 6.4 & 1.7 & 350.3 & Flat & 76.96$\pm$1.70 & 0.11$\pm$0.01  & 0.16$\times$0.15 & 128.1 & 31.4 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.020$\pm$0.000 & 0.039$\pm$0.003 & 2.8 & 0.07\\
HOPS-380   & \nodata & \nodata & HOPS-380  & 0.0 & HOPS-173-380 & 4.0 & 0.5 & 36.6 & 0    & 0.72$\pm$0.72 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-173-A & 05:36:26.041 & -06:25:05.09 & HOPS-173  & 0.1 & HOPS-173-380 & 7.3 & 0.8 & 60.2 & 0    & 4.66$\pm$0.66 & 0.04$\pm$0.01  & 0.11$\times$0.06 & 48.1 & 21.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.002$\pm$0.000 & 0.015$\pm$0.003 & 2.1 & 0.13\\
HOPS-173-B & 05:36:26.051 & -06:25:05.31 & HOPS-173  & 0.3 & HOPS-173-380 & 7.5 & 0.8 & 60.2 & 0    & 2.79$\pm$0.53 & 0.03$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.001$\pm$0.000 & 0.015$\pm$0.003 & 1.9 & 0.14\\
QSOJ0536225-0625136 & 05:36:22.551 & -06:25:13.63 & None      & -99.0 & HOPS-173-380 & 46.1 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 2.62$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 1.043$\pm$0.006 & -99.0 & -99.00\\
HOPS-199   & 05:34:39.887 & -06:25:14.02 & HOPS-199  & 0.4 & None      & -99.0 & 0.2 & 576.7 & Flat & 32.34$\pm$2.33 & -99.00$\pm$-99.00  & 0.91$\times$0.14 & 38.7 & 181.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.018$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-186   & 05:35:47.306 & -06:26:14.71 & HOPS-186  & 0.4 & HOPS-186  & 0.4 & 0.4 & 72.3 & I    & 56.63$\pm$1.86 & 0.21$\pm$0.04  & 0.51$\times$0.10 & 132.3 & 102.0 & 0.22$\times$0.10 & 131.1 & 43.2 & 0.023$\pm$0.001 & 0.104$\pm$0.020 & 2.4 & 0.10\\
HOPS-189   & 05:35:30.921 & -06:26:32.00 & HOPS-189  & 0.4 & HOPS-188  & 30.9 & 1.0 & 133.1 & I    & 5.33$\pm$0.57 & 0.03$\pm$0.03  & 0.08$\times$0.05 & 31.2 & 15.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.012$\pm$0.012 & 2.2 & 0.43\\
HOPS-188   & 05:35:29.844 & -06:26:58.13 & HOPS-188  & 0.4 & HOPS-188  & 0.4 & 15.7 & 103.3 & I    & 677.58$\pm$14.17 & 1.40$\pm$0.03  & 0.38$\times$0.22 & 75.0 & 76.4 & 0.11$\times$0.08 & 64.0 & 22.0 & 0.093$\pm$0.002 & 0.275$\pm$0.005 & 2.6 & 0.06\\
HOPS-190   & \nodata & \nodata & HOPS-190  & 0.0 & HOPS-188  & 20.1 & 0.3 & 385.3 & I    & 0.71$\pm$0.71 & 0.03$\pm$0.03  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.014$\pm$0.014 & 1.4 & 0.61\\
HOPS-172   & 05:36:19.463 & -06:29:06.91 & HOPS-172  & 0.3 & None      & -99.0 & 0.6 & 149.8 & I    & 11.06$\pm$0.71 & -99.00$\pm$-99.00  & 0.12$\times$0.08 & 105.2 & 23.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-379   & \nodata & \nodata & HOPS-379  & 0.0 & None      & -99.0 & 0.0 & 114.2 & I    & 0.68$\pm$0.68 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-170-B & 05:36:41.322 & -06:33:59.26 & HOPS-170  & 0.8 & None      & -99.0 & 2.1 & 832.5 & Flat & 49.73$\pm$1.66 & -99.00$\pm$-99.00  & 0.13$\times$0.12 & 144.6 & 25.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.012$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-170-A & 05:36:41.368 & -06:34:00.75 & HOPS-170  & 0.9 & None      & -99.0 & 2.1 & 832.5 & Flat & 72.40$\pm$1.82 & -99.00$\pm$-99.00  & 0.14$\times$0.14 & 167.0 & 28.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.018$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-197   & 05:34:15.897 & -06:34:32.66 & HOPS-197  & 0.2 & None      & -99.0 & 0.2 & 506.6 & Flat & 4.29$\pm$0.57 & -99.00$\pm$-99.00  & 0.06$\times$0.06 & 21.8 & 12.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-177   & 05:35:50.017 & -06:34:53.47 & HOPS-177  & 0.1 & None      & -99.0 & 0.4 & 84.7 & I    & 2.81$\pm$0.75 & -99.00$\pm$-99.00  & 0.19$\times$0.03 & 26.4 & 38.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-163-B & 05:37:17.329 & -06:36:18.10 & HOPS-163  & 0.7 & None      & -99.0 & 0.8 & 432.3 & I    & 1.70$\pm$0.25 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-163-A & 05:37:17.277 & -06:36:18.19 & HOPS-163  & 0.0 & None      & -99.0 & 0.8 & 432.3 & I    & 78.06$\pm$3.30 & -99.00$\pm$-99.00  & 0.79$\times$0.28 & 60.4 & 157.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.026$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-164   & 05:37:00.425 & -06:37:10.89 & HOPS-164  & 0.6 & HOPS-164  & 0.6 & 0.5 & 50.0 & 0    & 105.50$\pm$2.24 & 0.59$\pm$0.02  & 0.22$\times$0.14 & 150.8 & 43.2 & 0.10$\times$0.07 & 141.8 & 21.0 & 0.040$\pm$0.001 & 0.282$\pm$0.010 & 2.2 & 0.06\\
HOPS-171   & 05:36:17.208 & -06:38:01.51 & HOPS-171  & 0.2 & HOPS-171  & 0.2 & 1.5 & 61.8 & 0    & 30.64$\pm$1.07 & 0.17$\pm$0.02  & 0.30$\times$0.05 & 111.2 & 61.0 & 0.18$\times$0.04 & 105.8 & 37.0 & 0.008$\pm$0.000 & 0.061$\pm$0.008 & 2.2 & 0.08\\
HOPS-169   & 05:36:36.160 & -06:38:54.35 & HOPS-169  & 2.5 & HOPS-169  & 2.5 & 3.3 & 32.5 & 0    & 166.18$\pm$3.38 & 0.28$\pm$0.02  & 0.17$\times$0.13 & 61.5 & 33.0 & 0.09$\times$0.05 & 61.7 & 17.8 & 0.036$\pm$0.001 & 0.083$\pm$0.007 & 2.7 & 0.07\\
HOPS-166   & 05:36:25.131 & -06:44:41.83 & HOPS-166  & 0.1 & None      & -99.0 & 12.9 & 457.1 & Flat & 239.25$\pm$4.45 & -99.00$\pm$-99.00  & 0.16$\times$0.15 & 92.9 & 31.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.035$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-168-B & 05:36:18.952 & -06:45:23.48 & HOPS-168  & 0.8 & HOPS-168  & 0.8 & 40.0 & 54.0 & 0    & 42.05$\pm$3.05 & 0.75$\pm$0.02  & 0.13$\times$0.09 & 127.1 & 25.6 & 0.10$\times$0.04 & 4.8 & 20.8 & 0.004$\pm$0.000 & 0.116$\pm$0.004 & 1.7 & 0.07\\
HOPS-168-A & 05:36:18.941 & -06:45:23.58 & HOPS-168  & 0.9 & HOPS-168  & 0.9 & 40.0 & 54.0 & 0    & 140.11$\pm$2.27 & 1.15$\pm$0.02  & 0.07$\times$0.06 & 72.8 & 14.8 & 0.05$\times$0.04 & 151.9 & 10.8 & 0.015$\pm$0.000 & 0.179$\pm$0.003 & 2.1 & 0.06\\
QSOJ0536187-0625454 & 05:36:18.751 & -06:45:25.44 & HOPS-168  & 3.9 & HOPS-168  & 3.8 & -99.0 & -99.0 & \nodata & -99.00$\pm$-99.00 & 0.47$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.00$\times$0.00 & 0.0 & 0.0 & -99.000$\pm$-99.000 & 0.185$\pm$0.006 & -99.0 & -99.00\\
HOPS-167   & 05:36:19.808 & -06:46:00.82 & HOPS-167  & 0.2 & HOPS-168  & 40.3 & 0.1 & 568.6 & Flat & 2.07$\pm$0.40 & 0.05$\pm$0.05  & 0.05$\times$0.02 & 84.1 & 9.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & 0.033$\pm$0.033 & 1.6 & 0.44\\
HOPS-203-A & 05:36:22.865 & -06:46:06.63 & HOPS-203  & 0.6 & HOPS-203  & 0.6 & 17.0 & 43.7 & 0    & 61.73$\pm$1.10 & 0.99$\pm$0.02  & 0.18$\times$0.07 & 50.2 & 36.0 & 0.19$\times$0.05 & 142.9 & 38.0 & 0.008$\pm$0.000 & 0.191$\pm$0.004 & 1.8 & 0.06\\
HOPS-203-B & 05:36:22.862 & -06:46:06.75 & HOPS-203  & 0.7 & HOPS-203  & 0.7 & 17.0 & 43.7 & 0    & 7.87$\pm$0.33 & 0.14$\pm$0.01  & 0.00$\times$0.00 & 0.0 & 0.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.001$\pm$0.000 & 0.026$\pm$0.001 & 1.7 & 0.07\\
HOPS-203-C & 05:36:22.898 & -06:46:09.47 & HOPS-203  & 3.4 & HOPS-203  & 3.4 & 17.0 & 43.7 & 0    & 74.08$\pm$0.84 & 0.54$\pm$0.01  & 0.10$\times$0.06 & 175.4 & 19.0 & 0.06$\times$0.06 & 90.9 & 11.6 & 0.010$\pm$0.000 & 0.104$\pm$0.002 & 2.1 & 0.06\\
HOPS-165   & 05:36:23.539 & -06:46:14.52 & HOPS-165  & 0.0 & HOPS-203  & 13.3 & 2.8 & 96.1 & I    & 144.88$\pm$3.11 & 0.52$\pm$0.02  & 0.29$\times$0.12 & 95.2 & 59.0 & 0.10$\times$0.06 & 98.7 & 19.8 & 0.032$\pm$0.001 & 0.157$\pm$0.005 & 2.4 & 0.06\\
HOPS-378   & \nodata & \nodata & HOPS-378  & 0.0 & None      & -99.0 & 0.3 & 170.4 & I    & 0.71$\pm$0.71 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-159   & 05:37:53.764 & -06:47:17.07 & HOPS-159  & 0.4 & HOPS-160  & 40.7 & 0.4 & 498.4 & Flat & 2.06$\pm$0.49 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-160   & 05:37:51.056 & -06:47:20.64 & HOPS-160  & 0.3 & HOPS-160  & 0.3 & 1.2 & 80.4 & I    & 21.53$\pm$0.57 & 0.09$\pm$0.01  & 0.08$\times$0.02 & 70.4 & 15.2 & 0.02$\times$0.02 & 127.5 & 4.4 & 0.006$\pm$0.000 & 0.035$\pm$0.003 & 2.3 & 0.07\\
S13-038002 & \nodata & \nodata & S13-038002 & 0.0 & None      & -99.0 & -99.0 & -99.0 & \nodata & 0.72$\pm$0.72 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-355   & 05:37:17.123 & -06:49:49.12 & HOPS-355  & 0.7 & HOPS-355  & 0.7 & 1.0 & 44.9 & 0    & 16.26$\pm$0.65 & 0.11$\pm$0.02  & 0.08$\times$0.07 & 6.4 & 16.0 & 0.07$\times$0.04 & 127.1 & 14.2 & 0.005$\pm$0.000 & 0.046$\pm$0.007 & 2.1 & 0.09\\
HOPS-147   & \nodata & \nodata & HOPS-147  & 0.0 & None      & -99.0 & 0.1 & 619.6 & Flat & 0.57$\pm$0.57 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-157   & 05:37:56.574 & -06:56:39.47 & HOPS-157  & 0.3 & None      & -99.0 & 3.3 & 77.6 & I    & 58.87$\pm$3.32 & -99.00$\pm$-99.00  & 0.53$\times$0.46 & 15.8 & 105.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-156   & 05:38:03.430 & -06:58:15.89 & HOPS-156  & 0.4 & None      & -99.0 & 0.2 & 90.1 & I    & 11.37$\pm$0.57 & -99.00$\pm$-99.00  & 0.08$\times$0.05 & 24.7 & 16.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-149-B & 05:38:40.472 & -06:58:19.22 & HOPS-149  & 2.5 & None      & -99.0 & 9.9 & 484.6 & Flat & 72.82$\pm$3.31 & -99.00$\pm$-99.00  & 0.12$\times$0.11 & 39.6 & 24.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.012$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-149-A & 05:38:40.496 & -06:58:21.99 & HOPS-149  & 0.4 & None      & -99.0 & 9.9 & 484.6 & Flat & 289.47$\pm$6.21 & -99.00$\pm$-99.00  & 0.24$\times$0.22 & 49.7 & 48.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.047$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-158-A & 05:37:24.473 & -06:58:32.90 & HOPS-158  & 0.3 & None      & -99.0 & 2.3 & 591.6 & Flat & 4.21$\pm$0.45 & -99.00$\pm$-99.00  & 0.05$\times$0.01 & 37.6 & 10.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-158-B & 05:37:24.480 & -06:58:32.95 & HOPS-158  & 0.4 & None      & -99.0 & 2.3 & 591.6 & Flat & 4.39$\pm$0.51 & -99.00$\pm$-99.00  & 0.08$\times$0.02 & 71.1 & 16.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-154   & 05:38:20.113 & -06:59:04.78 & HOPS-154  & 0.3 & None      & -99.0 & 0.1 & 166.7 & I    & 2.86$\pm$0.87 & -99.00$\pm$-99.00  & 0.24$\times$0.11 & 12.3 & 47.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-148   & 05:38:39.523 & -06:59:30.23 & HOPS-148  & 0.2 & None      & -99.0 & 0.4 & 262.9 & I    & 1.63$\pm$0.49 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-142   & \nodata & \nodata & HOPS-142  & 0.0 & None      & -99.0 & 0.0 & 231.8 & I    & 0.62$\pm$0.62 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-143   & 05:38:46.193 & -07:00:48.47 & HOPS-143  & 0.2 & None      & -99.0 & 3.7 & 242.1 & I    & 15.63$\pm$0.48 & -99.00$\pm$-99.00  & 0.05$\times$0.02 & 25.8 & 9.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-141   & \nodata & \nodata & HOPS-141  & 0.0 & None      & -99.0 & 0.1 & 741.6 & Flat & 0.61$\pm$0.61 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-144   & 05:38:45.024 & -07:01:01.69 & HOPS-144  & 0.2 & None      & -99.0 & 1.9 & 99.2 & I    & 18.54$\pm$0.57 & -99.00$\pm$-99.00  & 0.10$\times$0.05 & 101.7 & 19.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-377   & 05:38:45.536 & -07:01:01.98 & HOPS-377  & 0.2 & None      & -99.0 & 3.3 & 53.7 & 0    & 19.77$\pm$0.94 & -99.00$\pm$-99.00  & 0.17$\times$0.09 & 145.2 & 33.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-145-B & 05:38:43.203 & -07:01:07.39 & HOPS-145  & 11.1 & None      & -99.0 & 1.8 & 133.7 & I    & 11.01$\pm$0.76 & -99.00$\pm$-99.00  & 0.11$\times$0.10 & 44.6 & 22.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-145-A & 05:38:43.851 & -07:01:13.10 & HOPS-145  & 0.2 & None      & -99.0 & 1.8 & 133.7 & I    & 35.93$\pm$0.72 & -99.00$\pm$-99.00  & 0.15$\times$0.05 & 40.9 & 30.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-139   & 05:38:49.626 & -07:01:17.63 & HOPS-139  & 0.2 & None      & -99.0 & 2.5 & 84.3 & I    & 20.50$\pm$0.70 & -99.00$\pm$-99.00  & 0.12$\times$0.05 & 28.7 & 24.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-140-C & 05:38:46.282 & -07:01:51.38 & HOPS-140  & 2.1 & None      & -99.0 & 0.5 & 137.2 & I    & 3.68$\pm$0.67 & -99.00$\pm$-99.00  & 0.14$\times$0.06 & 2.8 & 27.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-140-B & 05:38:46.274 & -07:01:53.62 & HOPS-140  & 0.2 & None      & -99.0 & 0.5 & 137.2 & I    & 101.53$\pm$5.91 & -99.00$\pm$-99.00  & 1.54$\times$0.58 & 72.2 & 308.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.039$\pm$0.002 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-140-A & 05:38:45.717 & -07:01:58.54 & HOPS-140  & 9.8 & None      & -99.0 & 0.5 & 137.2 & I    & 32.59$\pm$0.67 & -99.00$\pm$-99.00  & 0.12$\times$0.08 & 178.6 & 23.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-376   & 05:38:18.099 & -07:02:25.95 & HOPS-376  & 0.8 & HOPS-376  & 0.8 & 186.7 & 492.0 & Flat & 1199.52$\pm$25.55 & 0.88$\pm$0.02  & 0.37$\times$0.30 & 32.6 & 73.8 & 0.08$\times$0.06 & 19.7 & 16.8 & 0.087$\pm$0.002 & 0.095$\pm$0.002 & 3.1 & 0.06\\
HOPS-137   & \nodata & \nodata & HOPS-137  & 0.0 & None      & -99.0 & 0.1 & 43.7 & 0    & 0.62$\pm$0.62 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-138-A & 05:38:48.317 & -07:02:43.68 & HOPS-138  & 0.3 & None      & -99.0 & 0.1 & 42.8 & 0    & 4.87$\pm$0.63 & -99.00$\pm$-99.00  & 0.14$\times$0.08 & 78.6 & 29.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-138-B & 05:38:48.338 & -07:02:43.68 & HOPS-138  & 0.3 & None      & -99.0 & 0.1 & 42.8 & 0    & 0.97$\pm$0.19 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-136   & 05:38:46.529 & -07:05:37.41 & HOPS-136  & 0.1 & None      & -99.0 & 0.6 & 161.7 & I    & 73.80$\pm$2.46 & -99.00$\pm$-99.00  & 1.20$\times$0.11 & 113.8 & 240.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.027$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-153   & 05:37:57.023 & -07:06:56.27 & HOPS-153  & 0.3 & HOPS-153  & 0.3 & 3.8 & 39.4 & 0    & 148.10$\pm$3.00 & 0.64$\pm$0.02  & 0.39$\times$0.10 & 32.4 & 78.4 & 0.14$\times$0.05 & 34.1 & 27.4 & 0.031$\pm$0.001 & 0.184$\pm$0.007 & 2.3 & 0.06\\
HOPS-152   & 05:37:58.748 & -07:07:25.73 & HOPS-152  & 0.4 & HOPS-152  & 0.4 & 0.6 & 53.8 & 0    & 17.17$\pm$0.52 & 0.13$\pm$0.01  & 0.05$\times$0.04 & 86.0 & 10.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.006$\pm$0.000 & 0.061$\pm$0.006 & 2.1 & 0.07\\
HOPS-150-A & 05:38:07.530 & -07:08:29.01 & HOPS-150  & 0.2 & None      & -99.0 & 3.2 & 245.2 & Flat & 22.78$\pm$0.55 & -99.00$\pm$-99.00  & 0.05$\times$0.03 & 135.2 & 10.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-150-B & 05:38:07.530 & -07:08:32.23 & HOPS-150  & 3.0 & None      & -99.0 & 3.2 & 245.2 & Flat & 5.09$\pm$0.74 & -99.00$\pm$-99.00  & 0.09$\times$0.07 & 70.9 & 18.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-129   & 05:39:11.868 & -07:10:34.88 & HOPS-129  & 0.3 & None      & -99.0 & 1.5 & 191.3 & Flat & 54.86$\pm$1.02 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 44.5 & 19.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.016$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-133   & 05:39:05.834 & -07:10:39.24 & HOPS-133  & 0.1 & HOPS-133  & 0.1 & 2.9 & 74.6 & I    & 14.48$\pm$0.58 & 0.15$\pm$0.02  & 0.10$\times$0.04 & 6.3 & 19.8 & 0.09$\times$0.07 & 39.2 & 18.6 & 0.003$\pm$0.000 & 0.048$\pm$0.007 & 2.0 & 0.09\\
HOPS-131   & 05:39:07.579 & -07:10:52.22 & HOPS-131  & 0.2 & HOPS-133  & 29.0 & 0.1 & 82.3 & I    & 16.00$\pm$0.95 & 0.02$\pm$0.02  & 0.20$\times$0.10 & 12.1 & 40.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.010$\pm$0.001 & 0.016$\pm$0.016 & 2.8 & 0.43\\
HOPS-135   & 05:38:45.328 & -07:10:56.04 & HOPS-135  & 0.2 & None      & -99.0 & 1.0 & 130.3 & I    & 49.45$\pm$0.98 & -99.00$\pm$-99.00  & 0.11$\times$0.06 & 24.8 & 22.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.016$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-132   & 05:39:05.371 & -07:11:05.17 & HOPS-132  & 0.2 & HOPS-133  & 26.7 & 1.5 & 616.3 & Flat & 8.34$\pm$0.44 & 0.11$\pm$0.01  & 0.04$\times$0.02 & 122.9 & 7.8 & 0.03$\times$0.02 & 30.9 & 5.4 & 0.002$\pm$0.000 & 0.039$\pm$0.003 & 1.9 & 0.07\\
HOPS-134   & 05:38:42.791 & -07:12:43.82 & HOPS-134  & 0.2 & None      & -99.0 & 6.7 & 781.9 & Flat & 38.04$\pm$0.72 & -99.00$\pm$-99.00  & 0.06$\times$0.05 & 20.2 & 11.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.007$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-130   & 05:39:02.979 & -07:12:52.20 & HOPS-130  & 0.3 & None      & -99.0 & 1.3 & 156.7 & I    & 170.74$\pm$3.63 & -99.00$\pm$-99.00  & 0.46$\times$0.15 & 174.4 & 91.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.050$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-396   & \nodata & \nodata & HOPS-396  & 0.0 & None      & -99.0 & 0.0 & 58.7 & 0    & 0.69$\pm$0.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-122   & 05:39:45.139 & -07:19:13.43 & HOPS-122  & 0.2 & None      & -99.0 & 0.0 & 246.0 & I    & 7.62$\pm$1.08 & -99.00$\pm$-99.00  & 0.27$\times$0.11 & 9.9 & 53.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-127   & 05:39:00.972 & -07:20:22.55 & HOPS-127  & 0.5 & None      & -99.0 & 0.3 & 133.3 & I    & 8.93$\pm$0.46 & -99.00$\pm$-99.00  & 0.05$\times$0.03 & 36.7 & 9.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-375   & \nodata & \nodata & HOPS-375  & 0.0 & None      & -99.0 & 0.0 & 695.2 & I    & 0.72$\pm$0.72 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-128-A & 05:38:52.015 & -07:21:05.87 & HOPS-128  & 0.2 & None      & -99.0 & 0.7 & 469.2 & Flat & 14.18$\pm$0.58 & -99.00$\pm$-99.00  & 0.10$\times$0.05 & 84.7 & 20.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-128-B & 05:38:52.378 & -07:21:09.32 & HOPS-128  & 6.4 & None      & -99.0 & 0.7 & 469.2 & Flat & 11.37$\pm$0.54 & -99.00$\pm$-99.00  & 0.08$\times$0.06 & 103.7 & 16.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-123   & 05:39:33.286 & -07:22:57.45 & HOPS-123  & 0.2 & HOPS-121-123 & 4.3 & 0.4 & 50.1 & 0    & 88.23$\pm$2.07 & 0.20$\pm$0.02  & 0.26$\times$0.15 & 28.8 & 51.2 & 0.16$\times$0.05 & 23.2 & 32.4 & 0.039$\pm$0.001 & 0.109$\pm$0.012 & 2.6 & 0.08\\
HOPS-121   & \nodata & \nodata & HOPS-121  & 0.0 & HOPS-121-123 & 3.6 & 0.3 & 34.8 & 0    & 0.64$\pm$0.64 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-119   & 05:39:50.689 & -07:23:30.58 & HOPS-119  & 0.6 & None      & -99.0 & 1.0 & 573.8 & Flat & 2.49$\pm$0.63 & -99.00$\pm$-99.00  & 0.18$\times$0.06 & 67.5 & 35.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-408   & 05:39:30.904 & -07:23:59.67 & HOPS-408  & 2.3 & HOPS-408  & 2.3 & 0.5 & 37.9 & 0    & 90.36$\pm$2.49 & 0.21$\pm$0.02  & 0.28$\times$0.24 & 157.5 & 55.2 & 0.07$\times$0.05 & 141.4 & 13.0 & 0.037$\pm$0.001 & 0.109$\pm$0.009 & 2.6 & 0.07\\
HOPS-118   & 05:39:54.605 & -07:24:14.97 & HOPS-118  & 0.3 & None      & -99.0 & 0.3 & 552.8 & Flat & 3.39$\pm$0.50 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 73.7 & 19.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-117   & 05:39:55.460 & -07:24:19.48 & HOPS-117  & 0.3 & None      & -99.0 & 0.1 & 277.0 & Flat & 40.45$\pm$1.66 & -99.00$\pm$-99.00  & 0.37$\times$0.16 & 120.6 & 73.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.028$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-395-A & 05:39:17.092 & -07:24:24.55 & HOPS-395  & 2.5 & HOPS-395  & 2.5 & 0.4 & 31.7 & 0    & 12.19$\pm$0.61 & 0.21$\pm$0.03  & 0.02$\times$0.02 & 79.9 & 4.2 & 0.12$\times$0.08 & 88.6 & 23.2 & 0.005$\pm$0.000 & 0.111$\pm$0.014 & 1.7 & 0.08\\
HOPS-395-B & 05:39:17.081 & -07:24:24.57 & HOPS-395  & 2.4 & HOPS-395  & 2.4 & 0.4 & 31.7 & 0    & 4.98$\pm$0.61 & 0.24$\pm$0.02  & 0.02$\times$0.02 & 79.9 & 4.2 & 0.07$\times$0.04 & 51.6 & 14.8 & 0.002$\pm$0.000 & 0.123$\pm$0.009 & 1.3 & 0.09\\
HOPS-116   & 05:39:57.912 & -07:25:13.09 & HOPS-116  & 0.3 & None      & -99.0 & 0.3 & 411.1 & Flat & 22.62$\pm$0.72 & -99.00$\pm$-99.00  & 0.12$\times$0.06 & 139.8 & 23.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-114   & 05:40:01.391 & -07:25:38.76 & HOPS-114  & 0.3 & None      & -99.0 & 0.0 & 117.3 & I    & 3.75$\pm$0.50 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 10.5 & 20.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-115   & 05:39:56.542 & -07:25:51.62 & HOPS-115  & 0.6 & None      & -99.0 & 0.3 & 461.3 & Flat & 4.49$\pm$0.51 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 136.3 & 19.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-124   & 05:39:19.911 & -07:26:11.23 & HOPS-124  & 1.1 & HOPS-124  & 1.1 & 52.3 & 44.8 & 0    & 1232.89$\pm$25.04 & 1.45$\pm$0.03  & 0.35$\times$0.25 & 3.3 & 70.6 & 0.13$\times$0.09 & 73.7 & 25.2 & 0.131$\pm$0.003 & 0.227$\pm$0.005 & 2.9 & 0.06\\
HOPS-120   & 05:39:34.324 & -07:26:11.29 & HOPS-120  & 0.2 & None      & -99.0 & 0.3 & 455.3 & Flat & 3.39$\pm$0.66 & -99.00$\pm$-99.00  & 0.16$\times$0.10 & 93.5 & 32.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-125   & 05:39:19.540 & -07:26:17.13 & HOPS-125  & 2.0 & HOPS-124  & 8.9 & 8.6 & 110.5 & Flat & 13.42$\pm$1.95 & 0.25$\pm$0.02  & 0.07$\times$0.06 & 133.4 & 13.6 & 0.09$\times$0.04 & 20.3 & 17.8 & 0.002$\pm$0.000 & 0.061$\pm$0.005 & 1.7 & 0.09\\
HOPS-287   & 05:40:08.789 & -07:27:27.91 & HOPS-287  & 0.3 & None      & -99.0 & 0.7 & 117.8 & I    & 102.19$\pm$2.50 & -99.00$\pm$-99.00  & 0.39$\times$0.14 & 58.8 & 78.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.039$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-291   & 05:39:57.954 & -07:28:57.62 & HOPS-291  & 0.2 & HOPS-290  & 36.7 & 0.1 & 340.1 & Flat & 14.55$\pm$0.64 & 0.03$\pm$0.03  & 0.09$\times$0.06 & 153.7 & 18.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.000 & 0.021$\pm$0.021 & 2.7 & 0.43\\
HOPS-290-B & 05:39:57.329 & -07:29:32.71 & HOPS-290  & 1.4 & HOPS-290  & 1.4 & 1.7 & 47.3 & 0    & 69.14$\pm$2.25 & 0.03$\pm$0.01  & 0.50$\times$0.11 & 137.7 & 100.6 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.020$\pm$0.001 & 0.013$\pm$0.003 & 3.2 & 0.11\\
HOPS-285   & \nodata & \nodata & HOPS-285  & 0.0 & None      & -99.0 & 0.1 & 66.5 & 0    & 0.70$\pm$0.70 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-290-A & 05:39:57.377 & -07:29:33.10 & HOPS-290  & 0.6 & HOPS-290  & 0.6 & 1.7 & 47.3 & 0    & 27.44$\pm$1.02 & 0.14$\pm$0.01  & 0.10$\times$0.09 & 8.0 & 20.2 & 0.04$\times$0.02 & 57.3 & 8.4 & 0.008$\pm$0.000 & 0.053$\pm$0.005 & 2.3 & 0.08\\
HOPS-288-A-A & 05:39:56.001 & -07:30:27.57 & HOPS-288  & 0.9 & HOPS-288  & 0.9 & 126.3 & 48.6 & 0    & 902.37$\pm$19.14 & 1.34$\pm$0.02  & 0.42$\times$0.18 & 145.6 & 83.8 & 0.09$\times$0.07 & 99.7 & 17.2 & 0.079$\pm$0.002 & 0.174$\pm$0.003 & 2.8 & 0.06\\
HOPS-288-A-B & 05:39:56.006 & -07:30:27.70 & HOPS-288  & 0.9 & HOPS-288  & 1.0 & 126.3 & 48.6 & 0    & -99.00$\pm$-99.00 & 0.54$\pm$0.02  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.10$\times$0.06 & 135.9 & 20.2 & -99.000$\pm$-99.000 & 0.069$\pm$0.003 & -99.0 & -99.00\\
HOPS-288-B & 05:39:56.033 & -07:30:27.96 & HOPS-288  & 1.3 & HOPS-288  & 1.3 & 126.3 & 48.6 & 0    & 156.67$\pm$10.67 & 0.42$\pm$0.03  & 0.22$\times$0.10 & 121.2 & 44.2 & 0.11$\times$0.05 & 126.2 & 22.0 & 0.014$\pm$0.001 & 0.054$\pm$0.003 & 2.5 & 0.07\\
HOPS-286   & \nodata & \nodata & HOPS-286  & 0.0 & None      & -99.0 & 0.5 & 123.7 & I    & 0.69$\pm$0.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-282-A & 05:40:26.091 & -07:37:32.08 & HOPS-282  & 0.1 & None      & -99.0 & 0.8 & 95.1 & I    & 10.65$\pm$0.50 & -99.00$\pm$-99.00  & 0.04$\times$0.03 & 113.4 & 9.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-282-B & 05:40:26.080 & -07:37:32.10 & HOPS-282  & 0.2 & None      & -99.0 & 0.8 & 95.1 & I    & 1.88$\pm$0.44 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-281-A & 05:40:24.648 & -07:43:08.15 & HOPS-281  & 0.5 & None      & -99.0 & 1.3 & 189.3 & Flat & 66.24$\pm$1.27 & -99.00$\pm$-99.00  & 0.09$\times$0.08 & 103.9 & 17.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.022$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-281-B & 05:40:24.600 & -07:43:08.37 & HOPS-281  & 0.3 & None      & -99.0 & 1.3 & 189.3 & Flat & 1.28$\pm$0.46 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-276   & 05:40:42.924 & -07:45:01.98 & HOPS-276  & 0.2 & None      & -99.0 & 0.2 & 303.8 & I    & 2.78$\pm$0.44 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-279   & 05:40:17.806 & -07:48:25.84 & HOPS-279  & 0.3 & None      & -99.0 & 5.8 & 382.0 & Flat & 59.31$\pm$1.13 & -99.00$\pm$-99.00  & 0.10$\times$0.05 & 129.5 & 19.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.013$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-280   & 05:40:14.953 & -07:48:48.64 & HOPS-280  & 0.3 & None      & -99.0 & 3.2 & 121.2 & I    & 91.72$\pm$1.69 & -99.00$\pm$-99.00  & 0.13$\times$0.07 & 59.4 & 26.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.023$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-275   & 05:40:36.328 & -07:49:07.11 & HOPS-275  & 0.3 & None      & -99.0 & 0.1 & 146.4 & I    & 2.92$\pm$0.51 & -99.00$\pm$-99.00  & 0.10$\times$0.03 & 177.2 & 19.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-271   & \nodata & \nodata & HOPS-271  & 0.0 & None      & -99.0 & 0.1 & 108.4 & I    & 0.69$\pm$0.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-267   & 05:41:19.675 & -07:50:41.03 & HOPS-267  & 0.2 & None      & -99.0 & 1.1 & 186.2 & I    & 32.05$\pm$0.71 & -99.00$\pm$-99.00  & 0.06$\times$0.04 & 145.7 & 11.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.012$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-278   & 05:40:20.379 & -07:51:15.00 & HOPS-278  & 0.4 & None      & -99.0 & 0.2 & 96.3 & I    & 7.34$\pm$0.84 & -99.00$\pm$-99.00  & 0.14$\times$0.10 & 45.9 & 27.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-265   & 05:41:20.350 & -07:53:10.71 & HOPS-265  & 0.4 & None      & -99.0 & 0.1 & 635.1 & Flat & 12.50$\pm$0.75 & -99.00$\pm$-99.00  & 0.10$\times$0.10 & 20.1 & 20.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-266   & \nodata & \nodata & HOPS-266  & 0.0 & None      & -99.0 & 0.0 & 190.7 & Flat & 0.69$\pm$0.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-262   & 05:41:23.979 & -07:53:42.21 & HOPS-262  & 0.3 & None      & -99.0 & 0.9 & 202.4 & Flat & 14.67$\pm$0.60 & -99.00$\pm$-99.00  & 0.08$\times$0.07 & 66.7 & 15.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-263   & 05:41:23.691 & -07:53:46.76 & HOPS-263  & 0.1 & None      & -99.0 & 0.7 & 145.1 & I    & 35.74$\pm$1.12 & -99.00$\pm$-99.00  & 0.18$\times$0.15 & 103.9 & 35.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.015$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-253   & 05:41:28.784 & -07:53:51.04 & HOPS-253  & 0.2 & None      & -99.0 & 0.7 & 321.1 & Flat & 87.00$\pm$2.05 & -99.00$\pm$-99.00  & 0.19$\times$0.16 & 116.3 & 38.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.038$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-258   & 05:41:24.727 & -07:54:08.51 & HOPS-258  & 0.3 & None      & -99.0 & 1.1 & 385.7 & Flat & 46.29$\pm$1.12 & -99.00$\pm$-99.00  & 0.13$\times$0.09 & 128.1 & 25.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.017$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-270   & 05:40:40.560 & -07:54:39.77 & HOPS-270  & 0.4 & None      & -99.0 & 0.3 & 96.6 & I    & 1.48$\pm$0.60 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-274-A & 05:40:20.727 & -07:54:59.79 & HOPS-274  & 0.2 & None      & -99.0 & 1.9 & 546.5 & Flat & 1.60$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-274-B & 05:40:20.731 & -07:54:59.99 & HOPS-274  & 0.4 & None      & -99.0 & 1.9 & 546.5 & Flat & 1.21$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-254   & 05:41:24.518 & -07:55:07.41 & HOPS-254  & 0.1 & HOPS-254  & 0.1 & 6.2 & 114.7 & I    & 308.89$\pm$6.28 & 0.68$\pm$0.02  & 0.28$\times$0.16 & 120.3 & 56.2 & 0.09$\times$0.09 & 85.2 & 18.6 & 0.069$\pm$0.001 & 0.213$\pm$0.007 & 2.6 & 0.06\\
HOPS-374   & 05:41:25.459 & -07:55:18.80 & HOPS-374  & 0.1 & HOPS-254  & 18.1 & 0.2 & 56.9 & 0    & 2.45$\pm$0.65 & 0.04$\pm$0.04  & 0.17$\times$0.05 & 89.9 & 33.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.029$\pm$0.029 & 1.8 & 0.45\\
HOPS-261-A & 05:41:18.889 & -07:55:28.57 & HOPS-261  & 0.5 & None      & -99.0 & 2.4 & 149.5 & I    & 3.08$\pm$0.63 & -99.00$\pm$-99.00  & 0.13$\times$0.04 & 62.3 & 26.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-261-B & 05:41:18.894 & -07:55:29.34 & HOPS-261  & 0.3 & None      & -99.0 & 2.4 & 149.5 & I    & 3.72$\pm$0.75 & -99.00$\pm$-99.00  & 0.15$\times$0.07 & 68.2 & 29.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-257   & 05:41:19.897 & -07:55:46.77 & HOPS-257  & 0.4 & None      & -99.0 & 0.3 & 292.6 & Flat & 9.38$\pm$0.57 & -99.00$\pm$-99.00  & 0.07$\times$0.05 & 25.9 & 14.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-273   & 05:40:20.905 & -07:56:24.58 & HOPS-273  & 0.4 & None      & -99.0 & 2.2 & 243.3 & I    & 139.23$\pm$1.50 & -99.00$\pm$-99.00  & 0.25$\times$0.14 & 143.0 & 50.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.040$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-247   & 05:41:26.187 & -07:56:51.91 & HOPS-247  & 0.6 & HOPS-247  & 0.6 & 3.3 & 42.8 & 0    & 252.45$\pm$5.12 & 0.55$\pm$0.03  & 0.23$\times$0.16 & 17.9 & 46.6 & 0.10$\times$0.06 & 37.4 & 19.2 & 0.068$\pm$0.001 & 0.203$\pm$0.009 & 2.6 & 0.06\\
HOPS-248-B & 05:41:22.128 & -07:58:02.95 & HOPS-248  & 0.5 & None      & -99.0 & 2.2 & 484.3 & Flat & 2.02$\pm$0.38 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-248-A & 05:41:22.138 & -07:58:03.08 & HOPS-248  & 0.7 & None      & -99.0 & 2.2 & 484.3 & Flat & 45.82$\pm$0.94 & -99.00$\pm$-99.00  & 0.08$\times$0.06 & 35.7 & 16.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.014$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-245   & 05:41:22.892 & -07:58:56.00 & HOPS-245  & 0.5 & None      & -99.0 & 0.3 & 302.1 & Flat & 1.81$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-264   & 05:40:59.115 & -08:00:14.40 & HOPS-264  & 0.2 & None      & -99.0 & 0.1 & 402.3 & Flat & 1.13$\pm$0.42 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-268   & 05:40:38.357 & -08:00:36.03 & HOPS-268  & 0.4 & None      & -99.0 & 1.1 & 113.9 & I    & 5.77$\pm$1.39 & -99.00$\pm$-99.00  & 0.26$\times$0.16 & 42.2 & 51.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-239   & \nodata & \nodata & HOPS-239  & 0.0 & None      & -99.0 & 0.3 & 116.2 & I    & 0.71$\pm$0.71 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-241   & 05:41:26.453 & -08:01:02.08 & HOPS-241  & 0.8 & None      & -99.0 & 0.7 & 100.3 & I    & 14.26$\pm$0.57 & -99.00$\pm$-99.00  & 0.07$\times$0.04 & 37.9 & 13.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.006$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-240   & 05:41:25.988 & -08:01:15.85 & HOPS-240  & 0.3 & None      & -99.0 & 0.1 & 191.0 & I    & 2.24$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-233   & \nodata & \nodata & HOPS-233  & 0.0 & HOPS-234  & 35.3 & 0.0 & 106.2 & I    & 0.70$\pm$0.70 & 0.04$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.001 & 0.040$\pm$0.040 & 1.3 & 0.61\\
HOPS-234   & 05:41:49.961 & -08:01:26.27 & HOPS-234  & 0.3 & HOPS-234  & 0.3 & 2.4 & 79.8 & I    & 47.09$\pm$0.99 & 0.26$\pm$0.02  & 0.10$\times$0.05 & 110.9 & 20.4 & 0.06$\times$0.02 & 113.5 & 11.8 & 0.014$\pm$0.000 & 0.105$\pm$0.006 & 2.2 & 0.07\\
HOPS-284   & 05:38:51.499 & -08:01:27.46 & HOPS-284  & 0.3 & None      & -99.0 & 0.6 & 913.9 & Flat & 24.03$\pm$0.95 & -99.00$\pm$-99.00  & 0.15$\times$0.09 & 176.4 & 29.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-238   & 05:41:26.657 & -08:03:12.61 & HOPS-238  & 0.3 & None      & -99.0 & 0.4 & 269.1 & I    & 2.54$\pm$0.23 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-237   & 05:41:28.984 & -08:03:25.95 & HOPS-237  & 0.2 & None      & -99.0 & 0.3 & 177.7 & I    & 8.07$\pm$0.53 & -99.00$\pm$-99.00  & 0.06$\times$0.03 & 135.4 & 12.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-236   & 05:41:30.223 & -08:03:41.46 & HOPS-236  & 0.3 & None      & -99.0 & 5.2 & 332.8 & Flat & 97.71$\pm$2.03 & -99.00$\pm$-99.00  & 0.16$\times$0.11 & 172.6 & 31.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.023$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-251   & 05:40:54.017 & -08:05:13.18 & HOPS-251  & 0.2 & None      & -99.0 & 0.7 & 345.7 & Flat & 38.02$\pm$1.08 & -99.00$\pm$-99.00  & 0.18$\times$0.08 & 56.7 & 36.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.016$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-405   & 05:40:58.552 & -08:05:34.52 & HOPS-405  & 2.0 & HOPS-405  & 2.0 & 1.7 & 35.0 & 0    & 3.45$\pm$0.26 & 0.06$\pm$0.01  & 0.03$\times$0.01 & 173.3 & 6.0 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.001$\pm$0.000 & 0.027$\pm$0.003 & 1.7 & 0.08\\
HOPS-255-B & 05:40:50.567 & -08:05:48.57 & HOPS-255  & 0.1 & None      & -99.0 & 0.7 & 572.0 & Flat & 0.94$\pm$0.27 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-255-A & 05:40:50.576 & -08:05:48.70 & HOPS-255  & 0.1 & None      & -99.0 & 0.7 & 572.0 & Flat & 22.54$\pm$0.72 & -99.00$\pm$-99.00  & 0.09$\times$0.07 & 1.0 & 17.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.010$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-249   & 05:40:52.869 & -08:05:48.91 & HOPS-249  & 0.2 & None      & -99.0 & 0.1 & 268.5 & Flat & 28.25$\pm$1.19 & -99.00$\pm$-99.00  & 0.17$\times$0.14 & 58.6 & 34.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.025$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-235   & 05:41:25.354 & -08:05:54.70 & HOPS-235  & 0.2 & None      & -99.0 & 5.1 & 680.1 & Flat & 79.46$\pm$1.56 & -99.00$\pm$-99.00  & 0.11$\times$0.10 & 3.1 & 21.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.019$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-244   & 05:41:02.010 & -08:06:01.91 & HOPS-244  & 0.3 & HOPS-243-244 & 21.7 & 1.4 & 127.3 & I    & 83.46$\pm$1.83 & 0.28$\pm$0.03  & 0.26$\times$0.09 & 92.6 & 51.2 & 0.10$\times$0.07 & 59.1 & 20.2 & 0.028$\pm$0.001 & 0.126$\pm$0.012 & 2.4 & 0.07\\
HOPS-252   & 05:40:49.914 & -08:06:08.43 & HOPS-252  & 0.2 & None      & -99.0 & 1.9 & 329.2 & Flat & 3.32$\pm$0.56 & -99.00$\pm$-99.00  & 0.11$\times$0.06 & 108.3 & 21.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-256   & 05:40:45.274 & -08:06:42.20 & HOPS-256  & 0.3 & HOPS-256  & 0.3 & 0.1 & 72.4 & 0    & 2.97$\pm$0.65 & 0.02$\pm$0.02  & 0.13$\times$0.03 & 31.1 & 26.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & 0.017$\pm$0.017 & 2.1 & 0.44\\
HOPS-243   & 05:41:01.663 & -08:06:44.60 & HOPS-243  & 0.2 & HOPS-243-244 & 21.3 & 0.5 & 50.8 & 0    & 9.36$\pm$1.14 & 0.03$\pm$0.03  & 0.22$\times$0.20 & 104.1 & 44.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.005$\pm$0.001 & 0.018$\pm$0.018 & 2.5 & 0.44\\
HOPS-250   & 05:40:48.849 & -08:06:57.10 & HOPS-250  & 0.2 & HOPS-250  & 0.2 & 7.1 & 69.4 & 0    & 187.77$\pm$4.15 & 0.25$\pm$0.03  & 0.32$\times$0.19 & 43.4 & 64.4 & 0.15$\times$0.09 & 40.6 & 29.6 & 0.040$\pm$0.001 & 0.074$\pm$0.008 & 2.8 & 0.08\\
HOPS-250-B & 05:40:46.618 & -08:07:12.84 & None      & -99.0 & HOPS-250  & 36.5 & 7.1 & 69.4 & 0    & -99.00$\pm$-99.00 & 0.18$\pm$0.01  & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.06$\times$0.03 & 31.5 & 11.8 & -99.000$\pm$-99.000 & 0.055$\pm$0.003 & -99.0 & -99.00\\
HOPS-232   & 05:41:35.471 & -08:08:22.70 & HOPS-232  & 0.5 & None      & -99.0 & 1.2 & 187.9 & I    & 24.18$\pm$0.81 & -99.00$\pm$-99.00  & 0.12$\times$0.06 & 132.9 & 23.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-246   & 05:40:47.112 & -08:09:48.04 & HOPS-246  & 0.3 & None      & -99.0 & 0.4 & 95.6 & I    & 48.68$\pm$1.20 & -99.00$\pm$-99.00  & 0.17$\times$0.08 & 34.6 & 33.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.025$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-229   & \nodata & \nodata & HOPS-229  & 0.0 & None      & -99.0 & 0.4 & 471.6 & Flat & 0.65$\pm$0.65 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-242-A & 05:40:48.530 & -08:11:08.90 & HOPS-242  & 0.2 & None      & -99.0 & 0.7 & 836.7 & Flat & 7.42$\pm$0.57 & -99.00$\pm$-99.00  & 0.08$\times$0.04 & 93.2 & 15.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-242-B & 05:40:48.549 & -08:11:08.93 & HOPS-242  & 0.5 & None      & -99.0 & 0.7 & 836.7 & Flat & 2.80$\pm$0.25 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-259-A & 05:40:20.904 & -08:13:55.20 & HOPS-259  & 0.4 & None      & -99.0 & 0.8 & 410.3 & Flat & 10.53$\pm$0.51 & -99.00$\pm$-99.00  & 0.06$\times$0.04 & 66.7 & 12.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-259-B & 05:40:20.933 & -08:14:06.44 & HOPS-259  & 11.3 & None      & -99.0 & 0.8 & 410.3 & Flat & 4.56$\pm$0.25 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-260   & 05:40:19.400 & -08:14:16.29 & HOPS-260  & 0.1 & None      & -99.0 & 1.7 & 600.1 & Flat & 85.74$\pm$2.42 & -99.00$\pm$-99.00  & 0.38$\times$0.18 & 90.7 & 75.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.027$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-397   & 05:42:49.002 & -08:16:10.68 & HOPS-397  & 1.9 & HOPS-397  & 1.9 & 1.8 & 46.1 & 0    & 63.32$\pm$2.26 & 0.13$\pm$0.02  & 0.55$\times$0.14 & 131.6 & 109.0 & 0.07$\times$0.02 & 146.8 & 13.2 & 0.021$\pm$0.001 & 0.056$\pm$0.007 & 2.6 & 0.08\\
HOPS-223   & 05:42:48.491 & -08:16:34.68 & HOPS-223  & 0.5 & HOPS-397  & 24.6 & 20.4 & 247.5 & I    & 239.50$\pm$4.69 & 0.65$\pm$0.02  & 0.16$\times$0.15 & 44.4 & 32.4 & 0.09$\times$0.07 & 4.4 & 18.4 & 0.039$\pm$0.001 & 0.152$\pm$0.005 & 2.5 & 0.06\\
HOPS-221   & 05:42:47.067 & -08:17:06.91 & HOPS-221  & 0.2 & None      & -99.0 & 8.8 & 172.3 & I    & 194.42$\pm$3.46 & -99.00$\pm$-99.00  & 0.11$\times$0.10 & 19.4 & 22.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.040$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-215   & 05:43:09.583 & -08:29:27.23 & HOPS-215  & 0.1 & None      & -99.0 & 0.6 & 195.5 & I    & 8.95$\pm$0.69 & -99.00$\pm$-99.00  & 0.11$\times$0.07 & 17.7 & 22.8 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.004$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-216   & 05:42:55.566 & -08:32:48.36 & HOPS-216  & 0.5 & None      & -99.0 & 0.7 & 117.7 & I    & 20.46$\pm$0.86 & -99.00$\pm$-99.00  & 0.19$\times$0.04 & 20.7 & 37.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-228   & 05:41:34.183 & -08:35:27.87 & HOPS-228  & 0.3 & None      & -99.0 & 12.0 & 293.0 & I    & 76.66$\pm$1.51 & -99.00$\pm$-99.00  & 0.11$\times$0.08 & 107.3 & 22.2 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.015$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-214   & 05:42:47.232 & -08:36:36.88 & HOPS-214  & 0.3 & None      & -99.0 & 0.1 & 360.8 & Flat & 15.52$\pm$0.82 & -99.00$\pm$-99.00  & 0.17$\times$0.07 & 64.0 & 33.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.011$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-211   & 05:42:58.340 & -08:37:44.25 & HOPS-211  & 0.8 & None      & -99.0 & 0.3 & 87.9 & Flat & 3.50$\pm$0.54 & -99.00$\pm$-99.00  & 0.10$\times$0.06 & 3.8 & 19.6 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.002$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-227   & 05:41:32.340 & -08:37:55.54 & HOPS-227  & 0.1 & None      & -99.0 & 0.4 & 371.0 & Flat & 4.81$\pm$0.69 & -99.00$\pm$-99.00  & 0.16$\times$0.07 & 164.5 & 32.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.003$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-210   & 05:42:58.285 & -08:38:05.26 & HOPS-210  & 0.3 & None      & -99.0 & 1.4 & 204.9 & Flat & 95.13$\pm$2.15 & -99.00$\pm$-99.00  & 0.34$\times$0.09 & 12.3 & 69.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.033$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-213-B & 05:42:48.077 & -08:40:08.28 & HOPS-213  & 0.3 & None      & -99.0 & 1.6 & 534.9 & Flat & 1.61$\pm$0.48 & -99.00$\pm$-99.00  & 0.11$\times$0.00 & 84.9 & 21.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-213-A & 05:42:48.088 & -08:40:08.47 & HOPS-213  & 0.2 & None      & -99.0 & 1.6 & 534.9 & Flat & 2.45$\pm$0.42 & -99.00$\pm$-99.00  & 0.00$\times$0.00 & 0.0 & 0.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.001$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-226   & \nodata & \nodata & HOPS-226  & 0.0 & HOPS-224  & 29.1 & 0.9 & 350.2 & Flat & 0.72$\pm$0.72 & 0.04$\pm$0.04  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & 0.023$\pm$0.023 & 1.2 & 0.61\\
HOPS-224   & 05:41:32.066 & -08:40:09.77 & HOPS-224  & 0.6 & HOPS-224  & 0.6 & 3.3 & 48.6 & 0    & 252.61$\pm$5.38 & 0.24$\pm$0.04  & 0.29$\times$0.18 & 170.4 & 57.6 & 0.14$\times$0.09 & 13.5 & 27.0 & 0.071$\pm$0.002 & 0.093$\pm$0.014 & 3.0 & 0.09\\
HOPS-225   & 05:41:30.343 & -08:40:17.73 & HOPS-225  & 0.2 & HOPS-224  & 26.2 & 0.9 & 432.5 & Flat & 10.81$\pm$0.56 & 0.10$\pm$0.01  & 0.07$\times$0.03 & 6.0 & 13.8 & 0.03$\times$0.02 & 32.6 & 6.4 & 0.004$\pm$0.000 & 0.054$\pm$0.006 & 2.0 & 0.08\\
HOPS-209   & \nodata & \nodata & HOPS-209  & 0.0 & None      & -99.0 & 0.3 & 554.1 & I    & 0.69$\pm$0.69 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-220   & 05:41:29.786 & -08:42:46.21 & HOPS-220  & 0.2 & None      & -99.0 & 0.3 & 193.6 & I    & 24.54$\pm$0.84 & -99.00$\pm$-99.00  & 0.15$\times$0.05 & 3.8 & 29.4 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.014$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-219   & 05:41:29.289 & -08:43:04.31 & HOPS-219  & 0.6 & None      & -99.0 & 2.3 & 90.0 & I    & 71.48$\pm$1.39 & -99.00$\pm$-99.00  & 0.14$\times$0.06 & 87.1 & 29.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.022$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-208   & 05:42:52.733 & -08:44:13.11 & HOPS-208  & 0.5 & None      & -99.0 & 0.0 & 373.5 & Flat & 5.77$\pm$0.84 & -99.00$\pm$-99.00  & 0.20$\times$0.11 & 37.8 & 41.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.009$\pm$0.001 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-206   & 05:43:07.293 & -08:44:31.27 & HOPS-206  & 0.5 & HOPS-206  & 0.5 & 2.5 & 65.1 & 0    & 21.14$\pm$0.65 & 0.12$\pm$0.01  & 0.09$\times$0.04 & 18.9 & 17.8 & 0.00$\times$0.00 & 0.0 & 0.0 & 0.006$\pm$0.000 & 0.049$\pm$0.006 & 2.2 & 0.08\\
HOPS-204   & 05:43:10.185 & -08:46:07.86 & HOPS-204  & 0.1 & None      & -99.0 & 1.4 & 85.4 & I    & 61.69$\pm$1.10 & -99.00$\pm$-99.00  & 0.07$\times$0.06 & 87.0 & 15.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.022$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\
HOPS-207   & \nodata & \nodata & HOPS-207  & 0.0 & None      & -99.0 & 0.6 & 446.2 & Flat & 0.66$\pm$0.66 & -99.00$\pm$-99.00  & -99.00$\times$-99.00 & -99.0 & -19800.0 & -99.00$\times$-99.00 & -99.0 & -19800.0 & 0.000$\pm$0.000 & -99.000$\pm$-99.000 & -99.0 & -99.00\\


==> table-vla-data-short.tex <==
HH270VLA1-A & 05:51:34.587 & +02:56:46.03 & HH270VLA1 & 1.1 & HH270VLA1 & 2.3 & 0    & 0.243$\pm$0.019 & 0.166  & 7.5 & 0.08$\times$0.03 & 143.0\\
HH270VLA1-C & 05:51:34.595 & +02:56:45.89 & HH270VLA1 & 1.0 & HH270VLA1 & 2.2 & 0    & 0.530$\pm$0.029 & 0.212  & 7.5 & 0.11$\times$0.09 & 50.3\\
HH270VLA1-B & 05:51:34.601 & +02:56:45.89 & HH270VLA1 & 0.9 & HH270VLA1 & 2.2 & 0    & 0.088$\pm$0.006 & 0.160  & 7.5 & \nodata & \nodata\\
HH270mms1-B & 05:51:22.632 & +02:56:06.80 & HH270mms1 & 0.1 & HH270mms  & 13.4 & I    & $\leq$0.02 & $\leq$0.02  & 8.9 & \nodata & \nodata\\
HH270mms1-A & 05:51:22.717 & +02:56:04.98 & HH270mms1 & 2.2 & HH270mms  & 11.7 & I    & 0.907$\pm$0.025 & 0.463  & 8.2 & 0.09$\times$0.06 & 98.6\\
HH270mms2  & 05:51:22.572 & +02:55:43.16 & HH270mms2 & 0.4 & HH270mms  & 10.3 & Flat & $\leq$0.02 & $\leq$0.02  & 8.3 & \nodata & \nodata\\
HH111MMS-B & 05:51:46.066 & +02:48:30.81 & HH111mms  & 2.8 & HH111mms  & 3.0 & I    & 0.172$\pm$0.016 & 0.142  & 7.9 & 0.04$\times$0.02 & 82.0\\
HH111MMS-A & 05:51:46.253 & +02:48:29.64 & HH111mms  & 0.2 & HH111mms  & 0.0 & I    & 2.183$\pm$0.032 & 0.870  & 7.9 & 0.13$\times$0.09 & 7.5\\
HOPS-7     & 05:54:20.058 & +01:50:42.62 & HOPS-7    & 0.2 & HOPS-7    & 0.2 & 0    & 0.122$\pm$0.019 & 0.084  & 7.6 & 0.07$\times$0.06 & 149.5\\
HOPS-354   & 05:54:24.261 & +01:44:19.90 & HOPS-354  & 0.5 & HOPS-354  & 0.5 & 0    & 1.898$\pm$0.017 & 1.385  & 7.7 & 0.08$\times$0.03 & 61.3\\


==> table-vla-fields-short.tex <==
HH270VLA1    & 05:51:34.731 & +02:56:46.80 & 7.0 & 32.0 &  430.1 & 0    &  3\\
HH270mms     & 05:51:22.624 & +02:55:53.40 & 8.3 & 72.0 &  405.7 & I    &  1\\
HH111mms     & 05:51:46.253 & +02:48:29.63 & 23.0 & 78.0 &  410.6 & I    &  2\\
HOPS-7       & 05:54:20.045 & +01:50:42.75 & 0.5 & 58.0 &  357.1 & 0    &  1\\
HOPS-354     & 05:54:24.252 & +01:44:19.39 & 6.6 & 34.8 &  355.4 & 0    &  1\\
HOPS-1       & 05:54:12.336 & +01:42:35.49 & 1.5 & 72.6 &  356.9 & I    &  1\\
HOPS-406     & 05:47:43.361 & +00:38:22.45 & 0.5 & 24.6 &  430.3 & 0    &  3\\
HOPS-343     & 05:47:59.030 & +00:35:32.85 & 3.9 & 82.1 &  427.6 & I    &  1\\
HOPS-404     & 05:48:07.762 & +00:33:50.79 & 1.0 & 26.1 &  430.1 & 0    &  1\\
HOPS-340-341 & 05:47:01.071 & +00:26:22.24 & 1.9, 2.1 & 40.6, 39.4 &  430.9,  430.9 & 0   , 0    &  2\\


==> table-vla-obslog-short.tex <==
HOPS-310     &   1 & 2016 October 20    & 3C84, 3C48, J0541-0541\\
HOPS-400     &   1 & 2016 October 21    & 3C84, 3C48, J0552+0313\\
HH111mms     &   1 & 2016 October 22    & 3C84, 3C48, J0552+0313\\
HOPS-401     &   1 & 2016 October 23    & 3C84, 3C48, J0552+0313\\
HOPS-399/372 &   1 & 2016 October 23    & 3C84, 3C48, J0552+0313\\
HOPS-370     &   1 & 2016 October 26    & 3C84, 3C48, J0541-0541\\
HOPS-203     &   1 & 2016 October 27    & 3C84, 3C48, J0541-0541\\
HOPS-50      &   1 & 2016 October 27    & 3C84, 3C48, J0541-0541\\
HOPS-402     &   1 & 2016 October 29    & 3C84, 3C48, J0552+0313\\
HOPS-18      &   1 & 2016 October 29    & 3C84, 3C48, J0541-0541\\

